Stein Variational Adaptive Importance Sampling

We propose a novel adaptive importance sampling algorithm which incorporates Stein variational gradient decent algorithm (SVGD) with importance sampling (IS). Our algorithm leverages the nonparametric transforms in SVGD to iteratively decrease the KL divergence between our importance proposal and the target distribution. The advantages of this algorithm are twofold: first, our algorithm turns SVGD into a standard IS algorithm, allowing us to use standard diagnostic and analytic tools of IS to evaluate and interpret the results; second, we do not restrict the choice of our importance proposal to predefined distribution families like traditional (adaptive) IS methods. Empirical experiments demonstrate that our algorithm performs well on evaluating partition functions of restricted Boltzmann machines and testing likelihood of variational auto-encoders.

==> SteinIS 2/tex/background.tex <==
%\section{}
%We first give a brief introduction to Stein variational gradient descent (SVGD) \citep{liu2016stein},
%which we will leverage to design our nonparametric adaptive IS.
%where we will deploy the transformation defined in \citep{liu2016stein}  to design our nonparametric adaptive IS.
%Recent developments \citep{liu2016kernelized, oates2016control, chwialkowski2016kernel} introduce a set of fundamental techniques in Stein's method\citep{stein1986approximate} to practical machine learning. Our proposed method is rooted in the clever design leveraging the connection between kernelized Stein discrepancy(KSD) and the derivative of $\KL$ divergence by \citep{liu2016stein}.

%\subsection{Kernelized Stein Discrepancy}
%We first introduce the reproducing kernel Hilbert spaces(RKHS) and then discuss the advantages of KSD independently proposed by two groups of people \citet{liu2016kernelized} and \citet{chwialkowski2016kernel}.
%
%For a positive definite kernel $k(x,x'),$ its related RKHS $\mathcal{H}$ endowed with inner product $\langle\cdot, \cdot\rangle_\mathcal{H}$, any function $f(x)\in \mathcal{H}$ can be written as
%$$f(x)=\langle f(\cdot), k(\cdot, x)\rangle_\mathcal{H}, k(x,x')=\langle k(\cdot, x), k(\cdot, x')\rangle_\mathcal{H},$$
%which is termed as "reproducing" property. The inner product induces the norm $\|f\|_\mathcal{H}^2=f(\cdot), f(\cdot).$ The $d-$dimesional RKHS $\mathcal{H}^d=\mathcal{H}\times\cdots \mathcal{H}$, the Hilbert space of $d\times 1$ vector-valued functions $\bd{f}=\{f_l: f_l\in \mathcal{H}\}_{l\in[d]},$ is equipped with an inner product $\langle \bd{f}(\cdot), \bd{g}(\cdot)\rangle_{\mathcal{H}^d}=\sum_{l\in [d]}\langle f_l(\cdot), g_l(\cdot)\rangle$ and norm $\|\bd{f}\|_{\mathcal{H}^d}^2=\sum_l \|f_l\|_\mathcal{H}^2.$
%
%KSD is a new discrepancy for measuring differences between two probability distributions based on combing Stein's identity with the reproducing kernel Hilbert space theory. The KSD between two differential density functions $p(x)$ and $q(x)$ is defined as follows,
%\begin{equation}
%\label{ksdorigin}
% \mathbb{D}(q, p)=\mathbb{E}_{x,x'\sim q}[(\bd{s}_p(x)-\bd{s}_q(x))^T k(x, x')(\bd{s}_p(x')-\bd{s}_q(x'))],
%\end{equation}
%where $\bd{s}_p(x)$ is the score function of $p(x)$, $\bd{s}_p(x)=\nabla_x \log p(x).$ Equality (\ref{ksdorigin}) can be rewritten as
%\begin{equation}
% \mathbb{D}(q, p)=\mathbb{E}_{x,x'\sim q}[\kappa_p(x,x')],
%\end{equation}
%where $\kappa_p(x,x')$ is a positive kernel defined via
%\begin{equation}
%\label{ksdkernel}
%\begin{split}
%\kappa_p(x,x')=&\bd{s}_p(x)^\mathrm{T} k(x,x')\bd{s}_p(x')+\bd{s}_p(x)^\mathrm{T}\nabla_{x'}k(x,x')+\\
%&\bd{s}_p(x')^\mathrm{T}\nabla_x k(x,x')+\nabla_x\cdot(\nabla_{x'}k(x,x')).
%\end{split}
%\end{equation}
%$p=q$ if and only if $\mathbb{D}(q, p)=0.$ KSD maximizes the violation of Stein's identity in $\mathcal{H}^d$,
%\begin{equation}
%\label{ksdoptimal}
%\sqrt{ \mathbb{D}(q, p)}=\max_{\bd{f}\in \mathcal{H}^d}\mathbb{E}_{x\sim q(x)}[\mathrm{trace}(\bd{s_p}(x)+\nabla_x \bd{f}(x))].
%\end{equation}
%One advantage of KSD is that it does not require to evaluate the normalization constant of the target distributions which is required in KL divergence and difficult to calculate in complex models. Another advantage is that it can be widely applied even for the highly complex, structured graphical models and deep networks.
%\section{\normalsize{STEIN VARIATIONAL GRADIENT DESCENT}}
\section{STEIN VARIATIONAL GRADIENT DESCENT}
% \section{Stein Variational Gradient Descent}
We introduce the basic idea of Stein variational gradient descent (SVGD) and Stein discrepancy. 
The readers are referred to \citet{liu2016stein} and \cite{liu2016kernelized} for more detailed introduction.
%and
% SVGD is a nonparametric variational inference algorithm which evolves a set of particles $\{\bd{x}_i\}$   towards the target distribution $p(\bd x)$,  using iterative deterministic transforms that greedily decreases  the KL divergence objective function.
%_{i=1}^$ by%minimizing their $\KL$ divergence with the target distribution $p(\bd{x})$.

\paragraph{Preliminary}
We always assume $\vx=[x_1,\cdots, x_d]^\top \in \R^d$ in this paper.
Given a positive definite kernel $k(\vx,\vx')$, there exists an unique reproducing kernel Hilbert space (RKHS) $\H_0$,
formed by the closure of functions of form $f(\vx) = \sum_{i} a_i k(\vx,\vx_i)$ where $a_i \in \RR$, equipped with inner product
$\la f, ~ g\ra_{\H_0} = \sum_{ij}a_i k(\vx_i, \vx_j) b_j$ for $g(\vx) = \sum_j b_j k(\vx, \vx_j)$. 
Denote by $\H  = \H_0^d = \H_0 \times \cdots \times \H_0$ the vector-valued function space formed by $\vv f = [f_1, \ldots, f_d]^\top$, where $f_i \in \H_0$, $i=1,\ldots, d$, equipped with inner product $\la \vv f, ~ \vv g\ra_{\H}=\sum_{l=1}^d \la f_l, ~ g_l\ra_{\H_0}, $ for $\vv g =[g_1, \ldots, g_d]^\top.$ 
Equivalently, $\H$ is the closure of functions of form  $\vv f(\vx) = \sum_{i} \vv a_i k(\vx,\vx_i)$ where $\vv a_i \in \RR^d $ 
with inner product $\la \vv f, ~ \vv g\ra_{\H} = \sum_{ij}\vv a_i^\top \vv b_j k(\vx_i, \vx_j)$ for $\vv g(\vx) = \sum_{i} \vv b_i k(\vx,\vx_i)$. 
%and $\vv f =(f_1, f_2, \cdots, f_d)$. %%The   The induced norm is $\|\vv f\|_{\H}^2=\la \vv f, ~ \vv f\ra_{\H}.$
See e.g.,~\citet{berlinet2011reproducing} for more background on RKHS.  %\todo{cite [BOOK] Reproducing
 %kernel Hilbert spaces in probability and statistics
%and  Kernel Mean Embedding of Distributions: A Review and Beyonds, }

\subsection{Stein Discrepancy as Gradient of KL Divergence}
% \subsection{STEIN DISCREPANCY AS GRADIENT OF KL DIVERGENCE}
% \subsection{\normalsize{STEIN DISCREPANCY AS GRADIENT OF KL DIVERGENCE}}
%SVGD starts with a set of initial particles $\{\bd{x}_i^0 \colon i = 1,\ldots, N\}$, e.g., drawn from some simple distribution $q_0(\bd{x}),$
%At the $t$-th iteration, $it
%Assume we are interested in approximating a distribution with
Let $p(\vx)$ be a density function on $\R^d$ which we want to approximate. We assume that we know $p(\vx)$ only up to a normalization constant, that is,
\begin{equation}
\label{barp}
p(\vx) = \frac{1}{Z} \bar p(\vx), ~~~~~ Z = \int \bar p(\vx) d\vx,
\end{equation}
where we assume we can only calculate $\bar p(\vx)$ and $Z$ is a normalization constant (known as the partition function) that is intractable to calculate exactly.
We assume that $\log p(\vx)$ is differentiable w.r.t. $\vx$, and we have access to $\nabla \log p(\vx) = \nabla \log \bar p(\vx )$ which does not depend on $Z$.
%$\nabla \log p(\vx)$ is known
%$\n = \nabla \log \bar p(\vx )$

The main idea of SVGD is to use a set of sequential deterministic transforms
to iteratively push a set of particles $\{\vx_i\}_{i=1}^n$ towards the target distribution:
%iteratively update a set of particles $\{\vx_i\}$ by of form
%and updates the particles by iterative deterministic transforms of form,
%transform of form\
% \todo{fix $n$ vs. $N$}
 \begin{align}
 \label{update}
 \begin{split}
 & \vx_i \leftarrow  \T(\vx_i), ~~~~ \quad \forall i=1, 2,\cdots, n \\
& \T(\vx) =  \bd{x} +\epsilon \bd{\phi}(\bd{x}),
\end{split}
 \end{align}
 where we choose the transform $\T$ to be an additive perturbation by a velocity field  $\ff$,
 with a magnitude controlled by a step size
 $\epsilon$ that is assumed to be small. %is a step size that controls the magnitude of the transform,
%  and $\bd{\phi}(\bd{x})$ is a velocity field
 %steepest decent direction

The key question is the choice of the velocity field $\ff $; this is done by choosing $\ff$ to maximally decrease the $\KL$ divergence between the distribution of particles and the target distribution. Assume the current particles are drawn from $q$, and $\T\sharp q$ is the distribution of the updated particles, that is, $\T\sharp q$ is the distribution of
$\bd{\vx}'=\T(\vx) = \bd{\vx}+\epsilon\bd{\phi}(\bd{\vx})$ when $\vx \sim q$.
The optimal $\ff$ should solve the following functional optimization:
% this is framed as the
 \begin{align}
 \label{vgddecrease}
 \begin{split}
\mathbb{D}(q ~||~ p)  \overset{def}{=}  \max_{\bd{\phi} \in \mathcal \F  \colon  ||\ff ||_{\F}\leq 1 } \bigg\{ - \frac{d}{d\epsilon}\KL( \T\sharp q \mid\mid p)~ \big|_{\epsilon=0}  \bigg\},
%  \\&
%\hspace{-.1\textwidth}
%~~~~~~~~~~~~~~s.t. ~~  ||\ff ||_{\H}\leq 1 \bigg\},
\end{split}
 \end{align}
% where $\B $ is the unit ball of the function space $\mathcal{F.}$
% \begin{align}
% \label{vgddecrease}
% \begin{split}
%\S(q ~||~ p)  \overset{def}{=}
% \max_{\bd{\phi} \in \mathcal \H } \bigg\{  & - \frac{d}{d\epsilon}\KL( \T \sharp q \mid\mid p)~ \big|_{\epsilon=0}
%  \\&
%\hspace{-.1\textwidth}
%~~~~~~~~~~~~~~s.t. ~~  ||\ff ||_{\H}\leq 1 \bigg\},
%\end{split}
% \end{align}
% where $\T \sharp q$ denotes the distribution of the updated particles  $\bd{\vx}'=\T(\vx) = \bd{\vx}+\epsilon\bd{\phi}(\bd{\vx})$,
%when the density of the original particle $\bd{\vx}$ is $q$.
where $\mathcal{F}$ is a vector-valued normed function space that contains the set of candidate velocity fields $\ff$. 
%%a set of vector-valued functions

The maximum negative gradient value $\mathbb{D}(q ~||~ p)$ in \eqref{vgddecrease}
provides a discrepancy measure between two distributions $q$ and $p$ and is known as \emph{Stein discrepancy} \citep{gorham2015measuring, liu2016kernelized, chwialkowski2016kernel}: if $\mathcal{F}$ is taken to be large enough, we have $\mathbb{D}(q ~||~ p) = 0$ iff there exists no transform to further improve the KL divergence between $p$ and $q$, namely $p = q$.
%$p = q$ since there
%between $q$ and $p$,
%measure of the discrepancy
%$\T q$ is the pushforward measure of

It is necessary to use an infinite dimensional function space $\mathcal{F}$ to
obtain good transforms,
which then casts a challenging functional optimization problem.
%Although \eqref{vgddecrease} casts a functional optimization problem.
Fortunately, it turns out that a simple closed form solution can be obtained by taking
$\mathcal{F}$ to be an RKHS $\mathcal{H}=\mathcal{H}_0\times\cdots \mathcal{H}_0$,
where $\H_0$ is a RKHS of scalar-valued functions, associated with a positive definite kernel $k(x,x')$.
%Define . %with each $\mathcal{H}$ associated with a positive definite kernel $k(\bd{x}, \bd{x}')$,%We define $$\mathcal F = \{f\in \H^d \colon ~ ||f ||_{\H^d} \leq 1\}.$$
In this case, \citet{liu2016kernelized} showed that the optimal solution  of \eqref{vgddecrease} is $\ff^* / ||\ff^* ||_\H$, where
%yields the following simple form:
 \begin{equation}
 \label{transf}
 \bd{\phi}^*(\cdot)
 =\mathbb{E}_{\bd{x}\sim{q}}[\nabla_{\bd{x}} \log p(\bd{x})k(\bd{x},\cdot)+\nabla_{\bd{x}} k(\bd{x},\cdot)].
 \end{equation}
% In fact, the resulting  objective function, the maximum negative gradient of KL divergence,  coincides with a kernelized Stein discrepancy (KSD) measure between $q$ and $p$, that is,
%  \begin{equation}
% \label{optinball}
% \mathbb{D}(q_0, p) = \max_{\bd{\phi}\in \mathcal F} \bigg \{ - \frac{d}{d\epsilon}\KL(q_{[\epsilon\phi]}\mid\mid p)|_{\epsilon=0} \bigg\}.
% \end{equation}
In addition, the corresponding Stein discrepancy, known as kernelized Stein discrepancy (KSD) \citep{liu2016kernelized, chwialkowski2016kernel, gretton2009fast, oates2016control}, can be shown to have the following closed form
\begin{align}
\label{equ:sdefine}
\mathbb{D}(q ~||~ p) = ||\ff^* ||_\H =  \big(\mathbb{E}_{x,x'\sim q}[\kappa_p(\vx,\vx')]\big)^{1/2},
\end{align}
%his the kernelized Stein discrepancy (KSD) and
where $\kappa_p(x,x')$ is a positive definite kernel defined by
 \begin{align}
%\begin{split}
\kappa_p & (\bd{x},  \bd{x}') 
 = \bd{s}_p(\bd{x})^\top k(\bd{x},\bd{x}')\bd{s}_p(\bd{x}') + \bd{s}_p(\bd{x})^\top \nabla_{\bd{x}'}k(\bd{x},\bd{x}') \notag\\
% = \bd{s}_p(\bd{x})^\top k(\bd{x},\bd{x}')\bd{s}_p(\bd{x}') + \notag \\
% & +\bd{s}_p(\bd{x})^\top \nabla_{\bd{x}'}k(\bd{x},\bd{x}') \label{ksdkernel} \\
% &+\bd{s}_p(\bd{x}')^\top \nabla_{\bd{x}} k(\bd{x},\bd{x}')+\nabla_{\bd{x}}\cdot(\nabla_{\bd{x}'}k(\bd{x}, \bd{x}')). \notag
& +\bd{s}_p(\bd{x}')^\top \nabla_{\bd{x}} k(\bd{x},\bd{x}')+\nabla_{\bd{x}}\cdot(\nabla_{\bd{x}'}k(\bd{x}, \bd{x}')). \label{ksdkernel}
%\end{split}
\end{align}
where $\bd s_p(\vx) \overset{def}{=} \nabla \log p(\vx)$. %and is known as the score function of $p$.
We refer to \citet{liu2016kernelized} 
for the  derivation of \eqref{ksdkernel}, and further treatment of KSD in  
%More discussion about KSD can be found in 
\citet{chwialkowski2016kernel, oates2016control, gorham2017measuring}. 


%The optimal $ \bd{\phi}^*$  thereby is given as
% \begin{equation}
% \label{transf}
% \bd{\phi}^*(\cdot)=\mathbb{E}_{\bd{x}\sim{q_0}}[\nabla_{\bd{x}} \log p(\bd{x})k(\bd{x},\cdot)+\nabla_{\bd{x}} k(\bd{x},\cdot)].
% \end{equation}
 %\begin{equation}
% \frac{d}{d\epsilon}\KL(q_{[\epsilon\phi]}\mid\mid p)|_{\epsilon=0}=-\mathbb{E}_{\bd{x}\sim q}[\mathcal{T}_p\phi(x)],
% \end{equation}
% where $\mathcal{T}_p\bd{\phi}(\bd{x})=\nabla_{\bd{x}}\log p(\bd{x})^T\bd{\phi} + \nabla_{\bd{x}}\cdot \bd{\phi}.$
% When $\mathcal{F}$ is chosen as $\mathcal{H}^d=\mathcal{H}\times\cdots \mathcal{H},$ a vector-valued reproducing kernel Hilbert space(RKHS) with each $\mathcal{H}$ associated with a positive definite kernel $k(\bd{x}, \bd{x}'),$ \citet{liu2016stein} shows the optimization in (\ref{vgddecrease}) reduces to
% \begin{equation}
% \label{ksd}
% \bd{\phi}^*=\argmax_{\phi\in \mathcal{H}^d} \{\mathbb{E}_{\bd{x}\sim q}\mathbb{E}_{\bd{x}\sim q}[\mathcal{T}_p\phi(x)], \|\bd{\phi}\|_{\mathcal{H}^d}}\le 1 \}.
% \end{equation}
%\citet{liu2016kernelized} shows that the optimization problem (\ref{ksd}) has a closed-form solution,
%
%And the maximum in (\ref{ksd}) is actually the kernelized Stein discrepancy(KSD),
% \begin{equation}
% \mathbb{D}(q, p)=\mathbb{E}_{x,x'\sim q}[\kappa_p(x,x')],
%\end{equation}
%where $\kappa_p(x,x')$ is a positive kernel defined as
%\begin{equation}
%\label{ksdkernel}
%\begin{split}
%\kappa_p & (\bd{x},  \bd{x}')=\bd{s}_p(\bd{x})^\mathrm{T} k(\bd{x},\bd{x}')\bd{s}_p(\bd{x}')+\bd{s}_p(\bd{x})^\mathrm{T}\nabla_{\bd{x}'}k(\bd{x},\bd{x}')+\\
%&\bd{s}_p(\bd{x}')^\mathrm{T}\nabla_{\bd{x}} k(\bd{x},\bd{x}')+\nabla_{\bd{x}}\cdot(\nabla_{\bd{x}'}k(\bd{x}, \bd{x}')).
%\end{split}
%\end{equation}
%Equation (\ref{optinball}) indicates that when we choose the direction $\bd{\phi}$ as $\bd{\phi}^*$ and $\epsilon$ is infinitesimal, SVGD decreases the KL divergence between $q_{[\epsilon\bd{\phi}]}$ and $p(\bd{x})$ by $\epsilon \cdot \mathbb{D}(q_0, p)$, where $q_{[\epsilon\bd{\phi}]}$ is the density function of updated particles.
% \subsection{\normalsize{STEIN VARIATIONAL GRADIENT DESCENT}}
\subsection{Stein Variational Gradient Descent}
In order to apply the derived optimal transform in the practical SVGD algorithm, we approximate the expectation $\E_{\vx\sim q}[\cdot]$ in \eqref{transf} using  the empirical averaging of the current particles,
that is, given particles $\{\vx_i^\ell\}_{i=1}^n$ at the $\ell$-th iteration, we construct the following velocity field:
\begin{align}\label{equ:phit}
\!\!\! \!  \ff_{\ell+1}(\cdot ) =\frac{1}{n} \sum_{j=1}^n [\nabla \log p(\bd{x}_j^{\ell})k(\bd{x}_j^{\ell},\cdot)+\nabla_{\bd{x}_j^{\ell}} k(\bd{x}_j^{\ell},\cdot)].
\end{align}
The SVGD update at the $\ell$-th iteration is then given by
%\begin{align}\label{equ:svgdup2}
%\begin{split}
%\vx_i^{\ell+1}  \gets \T_{\ell+1}(\vx_{i}^{\ell}),  &\text{where}& 
% \T_{\ell+1}(\vx) =\vx + \epsilon \ff_{\ell+1}(\vx).
%\end{split}
%\end{align}
%
\begin{align}\label{equ:svgdup2}
\begin{split}
& \vx_i^{\ell+1}  \gets \T_{\ell+1}(\vx_{i}^{\ell}), \\
& \T_{\ell+1}(\vx) =\vx + \epsilon \ff_{\ell+1}(\vx).
\end{split}
\end{align}
Here transform $\T_{\ell+1}$ is adaptively constructed based on the most recent particles $\{\vx_i^\ell\}_{i=1}^n$.
%which pushes the particles towards the target distribution $p$.
 Assume the initial particles $\{\vx_i^0\}_{i=1}^n$ are i.i.d. drawn from some distribution $q_0$, then the pushforward maps of $\T_\ell$ define a sequence of distributions that bridges between $q_0$ and $p$:
\begin{align}\label{equ:qt}
q_{\ell} =  (\T_{\ell} \circ \cdots \circ \T_{1})\sharp q_0, \quad \ell=1, \ldots, K,
\end{align}
where $q_\ell$ forms increasingly better approximation of the target $p$ as $\ell$ increases.
Because $\{\T_\ell\}$ are nonlinear transforms,
$q_\ell$ can represent highly complex distributions even when the original $q_0$ is simple.
In fact, one can view $q_\ell$ as
a deep residual network \citep{he2016deep} constructed layer-by-layer in a fast, nonparametric fashion.

However,
because the transform $\T_{\ell}$ depends on the previous particles $\{\vx_{i}^{\ell-1}\}_{i=1}^n$ as shown in \eqref{equ:phit},
the particles $\{\vx_i^{\ell}\}_{i=1}^n$, after the zero-th iteration, depend on each other in a complex fashion,
%which introduces a complex dependency between the current particles  $\{x_i^{t}\}$, and makes
%the particles $\{x_i^{t}\}$
%which couples
%which it pushes through. This makes the particles $
%\{x_i^{t}\}$ depends on each other in a complex fashion,
and do not, in fact, straightforwardly follow distribution $q_{\ell}$ in \eqref{equ:qt}.
Principled approaches for analyzing such interacting particle systems can be found in~\citet[e.g.,][]{braun1977vlasov, spohn2012large, del2013mean, sznitman1991topics}. The goal of this work, however, is to provide a simple method to ``decouple'' the SVGD dynamics, transforming it into a standard 
importance sampling method that is amendable to easier analysis and interpretability, and also applicable to more general inference tasks such as estimating partition function of unnormalized distribution where SVGD cannot be applied.
%thing
%This fact makes it harder to analyze and interpret the result of SVGD, compared with typical Monte Carlo with i.i.d. samples.
%In this section, we describe a simple method to decouple generate i.i.d. samples from $q_t$.

%equipped with RBM
%is
% get
%One may expect that $q_t$ gets closer to $p$ as $t$ increases and hence form better approximation of $p$.
%develop an algorithm in practice, we approximate the expection

%However, SVGD just runs a set of particles to approximate the target distribution $p(\bd{x})$ for Bayesian inference and usually require a large number of iterations to diminish the approximation bias induced by these particles. And the particles evolved by SVGD are interactive and dependent with each other. Without keeping track of the intermediate distributions, the evolved particles cannot be applied to more general inference tasks such as estimating the partition functions of graphical models \citep{liu2015estimating, ma2013estimating} and the decoder-based generative models \citep{kingma2013auto, wu2016quantitative}. These concerns motivate us to introduce a new inference algorithm in the following.






==> SteinIS 2/tex/experiments.tex <==
% \section{\normalsize{EMPIRICAL EXPERIMENTS}}
\section{EMPIRICAL EXPERIMENTS}
\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[height=0.18\textwidth]{figures/KL.pdf} &
\includegraphics[height=0.18\textwidth]{figures/KSD.pdf} \\
{\small (a)  KL} &
{\small (b)  KSD}
\end{tabular}
\caption{GMM with 10 mixture components. $d=1.$ In SVGD, 500 particles are evolved. In SteinIS, $|A|=200$ and $|B|=500$. For SVGD and SteinIS, all particles are drawn from the same Gaussian distribution $q_0(\bd{x}).$}
\label{fig:KL}
\end{figure}

\begin{figure*}[t]
\centering
\begin{tabular}{cccc}
\includegraphics[height=0.19\textwidth]{figures/finalonex.pdf} &
\includegraphics[height=0.19\textwidth]{figures/finalonexx.pdf} &
\includegraphics[height=0.19\textwidth]{figures/finalonecosx.pdf} &
\includegraphics[height=0.19\textwidth]{figures/partition.pdf}
\raisebox{2em}{ \includegraphics[height=0.1\textwidth]{figures/legend.pdf}}\\
{\small (a)  $\mathbb{E}[x]$} &
{\small (b)  $\mathbb{E}[x^2]$ } &
{\small (c) $\mathbb{E}[\cos(w x + b)]$} &
{\small (d) Partition Function}\\
\end{tabular}
\caption{2D GMM with 10 randomly generated mixture components. (a)-(c) shows mean square error(MSE) for estimating $\mathbb{E}_p[h(x)],$ where $h(\bd{x})=x_j,~x_j^2,~\cos(wx_j+b)$ with $w\sim \normal(0,1)$ and $b\in \mathrm{Uniform}([0,1])$ for $j=1,2$, and the normalization constant (which is $1$ in this case). 
We used 800 transitions in SteinIS, HAIS and AIS, and take $L=1$ in HAIS. We fixed the size of the leader particles $|A|$ to be $100$ and vary the size of follower particles $|B|$ in SteinIS. The initial proposal $q_0$ is the standard Gaussian. "Direct" means that samples are directly drawn from $p$ and is not applicable in (d). "IS" means we directly draw samples from $q_0$ and apply standard importance sampling. "Path" denotes  path integration method in Algorithm~\ref{ksdalgo} and is only applicable to estimate the partition function in (d). The MSE is averaged on each coordinate over 500 independent experiments for SteinIS, HAIS, AIS and Direct, and over 2000 independent experiments for IS. SVGD has similar results (not shown for clarity) as our SteinIS on (a), (b), (c), but can not be applied to estimate the partition function in task (d). 
%and is not provided in this figure for clarity. SVGD cannot be applied to task (d). 
The logarithm base is 10.
}
\label{fig:varyparticle}
\end{figure*}

We study the empirical performance of our proposed algorithms on both simulated and real world datasets. 
We start with toy examples to numerically investigate some theoretical properties of our algorithms, 
and compare it with traditional adaptive IS on non-Gaussian, multi-modal distributions. 
%Then we compare the empirical performance of our algorithm and traditional adaptive IS on non-Gaussian %on a probability model, which is not from the Gaussian mixture family. 
We also employ our algorithm to estimate the partition function of Gaussian-Bernoulli Restricted Boltzmann Machine(RBM), a graphical model widely used in deep learning~\citep{welling2004exponential, hinton2006reducing}, and to evaluate the log likelihood of decoder models in variational autoencoder~\citep{kingma2013auto}.

We summarize some hyperparameters used in our experiments. We use RBF kernel $k(\bd{x}, \bd{x}')=\exp(-\|\bd{x}-\bd{x}'\|^2/h),$ where $h$ is the bandwidth. In most experiments, we let $h {=} \mathrm{med^2}/(2\log(|A|+1))$, where $\mathrm{med}$ is the median of the pairwise distance of the current leader particles $\vx_A^\ell$, 
and $|A|$ is the number of leader particles. 
 %except for the evaluation of deep generative model. When evaluating the deep generative model, we use $h=0.9\cdot h_0+0.1\cdot h_0^2.$ 
 The step sizes in our algorithms are chosen to be $\epsilon =\alpha/(1+\ell)^\beta,$ where $\alpha$ and $\beta$ are hyperparameters chosen from a validation set to achieve best performance. When $\epsilon\le 0.1$, we use first-order approximation to calculate the determinants of Jacobian matrices as illustrated in proposition~\ref{detapprox}.

%We clarify some notations. 
In what follows, 
we use ``{AIS}'' to refer to the annealing importance sampling with Langevin dynamics as its Markov transitions, and use ``{HAIS}'' to denote the annealing importance sampling whose Markov transition is Hamiltonian Monte Carlo (HMC). %As mentioned in the introduction, the distribution path $\{q_\ell\}$ in SteinIS which bridge the target $p$ to $q_0$ is contrastive to the annealing path in AIS. 
We use "transitions" to denote the number of intermediate distributions constructed in the paths of both SteinIS and AIS. 
A transition of HAIS may include $L$ leapfrog steps, as implemented by ~\citet{wu2016quantitative}. 

% \vspace{-0.4cm}
% \subsection{\normalsize{GAUSSIAN MIXTURES MODLE (GMM)}}
 \subsection{Gaussian Mixtures Models}
 We start with testing our methods on simple 2 dimensional Gaussian mixture models (GMM) with 10 randomly generated mixture components. 
First, we numerically investigate the convergence of KL divergence between the particle distribution $q_t$ (in continuous time) and $p.$ Sufficient particles are drawn and infinitesimal step $\epsilon$ is taken to closely simulate the continuous time system, as defined by \eqref{part}, \eqref{diffode} and \eqref{klksd}. Figrue~\ref{fig:KL}(a)-(b) show that the KL divergence $\KL(q_t, p)$, 
 as well as the squared Stein discrepancy $\mathbb{D}(q_t, p)^2$, seem to decay exponentially in both SteinIS and the original SVGD. 
 This suggests that the quality of our importance proposal $q_t$ improves quickly as we apply sufficient transformations. However, it is still an open question to establish the exponential decay theoretically; 
 see \citet{liu2017stein} for a related discussion. 
%  is a good proposal for implementing IS as long as sufficient transformations are implemented to ensure that $\KL(q_t, p)$ decreases to be sufficiently small.
 %between the particle distribution $q_t(\bd{x})$ and the target distribution $p(\bd{x})$ satisfies $\KL(q_t, p)\propto \exp(-\gamma_1 t).$  The negative of its derivative $\mathbb{S}(q_t, p)^2$ in \eqref{klksd}, also has the exponential decay,  $\mathbb{S}(q_t, p)^2\propto \exp(-\gamma_2 t),$ as indicated by Figrue~\ref{fig:KL}(b).  
% And we have $|\gamma_1-\gamma_2|<0.002$ in our experiment. These results give us the conjecture that $\KL(q_t, p)=C\exp(-\gamma t)$ and $\mathbb{S}(q_t, p)^2 =C\gamma\exp(-\gamma t)$ although their analytical solutions are not available. 
%These results numerically indicate that $\KL(q_t, p)$ has exponential decays on GMM and validate that our importance proposal $q_t(\bd{x})$ is a good proposal for implementing IS as long as sufficient transformations are implemented to ensure that $\KL(q_t, p)$ decreases to be sufficiently small.

We also empirically verify the convergence property of our SteinIS 
as the follower particle size $|B|$ increases (as the leader particle size $|A|$ is fixed). We apply SteinIS to estimate $\mathbb{E}_p[h(x)],$ where $h(\bd{x})=x_j,~x_j^2 ~\textit{or}~\cos(wx_j+b)$ with $w \sim \normal(0,1)$ and $b \sim \mathrm{Uniform}([0,1])$ for $j=1,2$, and the partition function (which is trivially $1$ in this case). From Figure~\ref{fig:varyparticle}, we can see that the mean square error(MSE) of our algorithms follow the typical convergence rate of IS, which is $O(1/\sqrt{|B|}),$ where $|B|$ is the number of samples for performing IS. Figure~\ref{fig:varyparticle} indicates that SteinIS can achieve almost the same performance as the exact Monte Carlo~(which directly draws samples from the target $p$), 
indicating the proposal $q_\ell$ closely matches the target $p$. 
%when enough transformations are implemented to ensure that our importance proposal $q_\ell$ approximately matches $p$.

\begin{figure*}[t]
\centering
\scalebox{.99}{
\setlength{\tabcolsep}{0em}
\begin{tabular}{cccc}
\hspace{-.5cm} \includegraphics[height=0.22\textwidth]{figures/S1.pdf}&
\includegraphics[height=0.22\textwidth]{figures/S2.pdf} &
\includegraphics[height=0.22\textwidth]{figures/S3.pdf} &
\includegraphics[height=0.22\textwidth]{figures/S4.pdf} \\
{\small (a) SteinIS, $\ell=0$} & {\small (b) SteinIS,  $\ell=50$ } & {\small (c)  SteinIS, $\ell=200$} & {\small (d) SteinIS,  $\ell=2000$ } \\
\hspace{-.5cm} \includegraphics[height=0.21\textwidth]{figures/ada0.pdf} &
\includegraphics[height=0.21\textwidth]{figures/ada1.pdf} &
\includegraphics[height=0.21\textwidth]{figures/ada2.pdf} &
\includegraphics[height=0.21\textwidth]{figures/exact.pdf} \\
{\small (e) Adap IS, 0 iteration} & {\small (f) Adap IS, 1000 iteration } & {\small (g) Adap IS, 10000 iteration} & {\small (h)  Exact } \\
\end{tabular}
}
\caption{Evolution of the contour of density functions for SteinIS and Adaptive IS. The top row (a)-(d) shows the contours of the evolved density functions in SteinIS, and bottom row (c)-(g) are the evolved contours of the traditional adaptive IS with Gaussian mixture proposals. (h) is the contour of the target density $p$. The number of the mixture components for adaptive IS is $200$ and the number of leader particles for approximating the map in SteinIS is also $200$. }
\label{fig:adap}
\end{figure*}
\subsection{Comparison between SteinIS and Adaptive IS}
In the following, we compare SteinIS with traditional adaptive IS~\citep{ryu2014adaptive} on a probability model $p(\bd{x})$, obtained by applying nonlinear transform on a three-component Gaussian mixture model. % defined as $\widetilde{q}(\bd{z})=\sum_{k=1}^3\alpha_k \mathcal{N}(\bd{z};\bd{\mu}_k, \mathbf{\Sigma}_k)$. 
Specifically, let $ \widetilde{q}$ be a 2D Gaussian mixture model, and 
$\bd T$ is a nonlinear transform defined by $\bd{T}(\bd{z})=[a_1z_1+b_1, a_2 z_1^2+a_3z_2+b_2]^{\top}$, where $\bd{z}=[z_1, z_2]^{\top}.$ We define the target $p$ to be the distribution of $\vx  = \bd T (\bd z)$ when $\bd z \sim \widetilde q$. 
%we apply nonlinear transform $\vx=\bd{T}(\bd{z}),$ where $\bd{z}\sim \widetilde{q}(\bd{z}),$ to get the target $p(\bd{x})$.  The nonlinear transform is defined as $\bd{T}(\bd{z})=(a_1z_1+b_1, a_2 z_1^2+a_3z_2+b_2)^{\top}$, where $\bd{z}=(z_1, z_2)^{\top}.$ 
The contour of the target density $p$ we constructed is shown in Figure~\ref{fig:adap}(h). 
We test our SteinIS with $|A| = 100$ particles 
and visualize in Figure~\ref{fig:adap}(a)-(d) the density of the evolved distribution $q_\ell$ using kernel density estimation, by drawing a large number of follower particles. 
We compare our method with 
the adaptive IS by \citep{ryu2014adaptive} 
using a proposal family formed by Gaussian mixture with $200$ components. 
The densities of the proposals obtained by adaptive IS at different iterations
are shown in Figure~\ref{fig:adap}(e)-(g). 
%
%
We can see that the evolved proposals of SteinIS converge to the target density $p(\bd{x})$ and approximately match $p(\bd{x})$ at 2000 iterations, but the optimal proposal of adaptive IS with 200 mixture components (at the convergence) can not fit $p(\bd{x})$ well, as indicated by Figure~\ref{fig:adap}(g). This is because the Gaussian mixture proposal family (even with upto 200 components) can not closely approximate the non-Gaussian target distribution we constructed. 
We should remark that SteinIS can be applied to refine 
the optimal proposal given by adaptive IS to get better importance proposal by implementing a set of successive transforms on the given IS proposal. 

Qualitatively, we find that the KL divergence (calculated via kernel density estimation) between our evolved  proposal $q_\ell$ and $p$ decreases to  $\leq 0.003$ after 2000 iterations, while the KL divergence between the optimal adaptive IS proposal  and the target $p$ can be only decreased to $0.42$ even after sufficient optimization. 
% From Figure~\ref{fig:adap}(a) to ~\ref{fig:adap}(d), 

 
\begin{figure}[h]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.2\textwidth]{figures/GauBerDim.pdf} &
\includegraphics[width=0.2\textwidth]{figures/GauBer100.pdf} \\
{\small (a)  Vary dimensions} &
{\small (b)  100 dimensions}
\end{tabular}
\caption{Gauss-Bernoulli RBM with $d'=10$ hidden variables. The initial distribution $q_0(\bd{x})$ for all the methods  is a same multivariate Gaussian. We let $|A|=100$ in SteinIS and use $(B=)$100 importance samples in SteinIS, HAIS and AIS. In (a), we use 1500 transitions for HAIS, SteinIS and AIS. "HAIS-1L" means we use $L=1$ leapfrog in each Markov transition of HAIS. 
$\log Z^*$ denotes the logarithm of the exact normalizing constant. All experiments are averaged over 500 independent trails. 
%SVGD is not applicable. 
}
\label{fig:GauBerlli}
\end{figure}
% \subsection{GAUSS-BERNOULLI RESTRICTED BOLTZMANN MACHINE (RBM)}
% \subsection{\normalsize{GAUSS-BERNOULLI RESTRICTED BOLTZMANN MACHINE (RBM)}}
\subsection{Gauss-Bernoulli Restricted Boltzmann Machine}
%In this subsection, we test our SteinIS in a multi-modal model. 
We apply our method to estimate the partition function of Gauss-Bernoulli Restricted Boltzmann Machine (RBM), which is a multi-modal, hidden variable graphical model. It consists of a continuous observable variable $\bd{x}\in \mathbb{R}^d$ and a binary hidden variable $\bd{h}\in \{\pm 1\}^{d'},$ with a joint probability density function of form 
\begin{equation}
p(\bd{x},\bd{h})= \frac{1}{Z} \exp(\bd{x}^\mathrm{T} B\bd{h}+b^\mathrm{T}\bd{x}+c^\mathrm{T}\bd{h}-\frac{1}{2}\| \bd{x}\|_2^2),
\end{equation}
where $p(\bd{x})=\frac{1}{Z}\sum_{\bd{h}} p(\bd{x},\bd{h})$ and $Z$ is the normalization constant. 
By marginalzing the hidden variable $h$, we can show that $p(\bd{x})$ is 
%We can show $p(\bd{x})$ is given as
\begin{equation*}
\begin{aligned}
p(\bd{x})=\frac{1}{Z}\exp(b^\mathrm{T}\bd{x}-\frac12\| \bd{x}\|_2^2)\prod_{i=1}^{d'} [\exp(\varphi_i)+ \exp(-\varphi_i)],
\end{aligned}
\end{equation*}
where $\varphi = B^\mathrm{T}\bd{x} + c$, and its score function $\bd{s}_p$ is easily derived as
$$
\bd{s}_p(\bd{x})  = \nabla_{\bd x} \log p(\bd x) = b - \bd{x} + B\frac{\exp(2\varphi)-1}{\exp(2\varphi)+1}.
$$

In our experiments, we simulate a true model $p(\bd{x})$ by drawing $b$ and $c$ from standard Gaussian and select $B$ uniformly random from $\{0.5, -0.5\}$ with probability 0.5. The dimension of the latent variable $\bd{h}$ is 10 so that the probability model $p(\bd{x})$ is the mixture of  $2^{10}$ multivariate Gaussian distribution. The exact normalization constant $Z$ can be feasibly calculated using the brute-force algorithm in this case. 
Figure~\ref{fig:GauBerlli}(a) and Figure \ref{fig:GauBerlli}(b) shows the performance of SteinIS on Gauss-Bernoulli RBM 
when we vary the dimensions of the observed variables 
and the number of transitions in SteinIS, respectively.  
%and \ref{fig:GauBerlli}(b) shows the result 
 %and 100-dimensional observed variable respectively. 
 We can see that SteinIS converges slightly faster than HAIS which uses one leapfrog step in each of its Markov transition. Even with the same number of Markov transitions, AIS with Langevin dynamics converges much slower than both SteinIS and HAIS. 
The better performance of HAIS comparing to AIS was also observed by ~\citet{sohl2012hamiltonian} when they first proposed HAIS. 

\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.2\textwidth]{figures/decode20.pdf}&
\includegraphics[width=0.2\textwidth]{figures/decode50.pdf} \\
{\small (a)  20 hidden variables}&
{\small (b)  50 hidden variables}
\end{tabular}
\caption{
Calculating the testing log-likelihood $\log p(x)$ for the deep generative model on MNIST. 
The initial distribution $q_0$ used in SteinIS, HAIS and AIS is a same multivariate Gaussian. 
We let $|A|=60$ in SteinIS and use 60 samples for each image to implement IS in HAIS and AIS. "HAIS-10L" and "HAIS-1L" denote using $L=10$ and $L=1$ in each Markov transition of HAIS, respectively. The log-likelihood $\log p(x)$ is averaged over 1000 images randomly chosen from MNIST. 
Figure (a) and (b) show the results when using $20$ and $50$ hidden variables, respectively. 
Note that the dimension of the observable variable $\vx$ is fixed, and is the size of the MNIS images. }
%The dimensions in (a) and (b) are the dimensions of latent space $\bd{z}$ in our setting.}
\label{figdecode}
\end{figure}
% \subsection{DEEP GENERATIVE MODELS}
% \subsection{\normalsize{DEEP GENERATIVE MODELS}}
\subsection{Deep Generative Models}
 Finally, we implement our SteinIS to evaluate the $\log$-likelihoods of the decoder models in variational autoencoder (VAE) \citep{kingma2013auto}. VAE is a directed probabilistic graphical model. The decoder-based generative model is defined by a joint distribution over a set of latent random variables $\bd{z}$ and the observed variables $\bd{x}: p(\bd{x}, \bd{z})=p(\bd{x}\mid \bd{z}) p(\bd{z}).$ We use the same network structure as that in \citet{kingma2013auto}. The prior $p(\bd{z})$ is chosen to be a multivariate Gaussian distribution. The log-likelihood is defined as $p(\bd{x})=\int p(\bd{x}\mid\bd{z})p(\bd{z})d\bd{z},$ where $p(\bd{x}\mid \bd{z})$ is the Bernoulli MLP as the decoder model given in \citet{kingma2013auto}.
 In our experiment, we use a two-layer network for $p(\bd{x}\mid\bd{z}),$ whose parameters are estimated using a standard VAE based on the MNIST training set.  
 For a given observed test image $\vx$, we use our method to sample the posterior distribution $p(\bd z | \vx)  = \frac{1}{p(\vx)}  p(\bd{x} | \bd{z}) p(\bd{z})$, and estimate the partition function $p(x)$, which is the testing likelihood of image $\vx$. 

Figure~\ref{figdecode} also indicates that our SteinIS converges slightly faster than HAIS-1L which uses one leapfrog step in each of its Markov transitions, denoted by HAIS-1L. Meanwhile, the running time of SteinIS and HAIS-1L is also comparable as provided by Table~\ref{timetable}. Although HAIS-10L, which use 10 leapfrog steps in each of its Markov transition, converges faster than our SteinIS, it takes much more time than our SteinIS in our implementation since the leapfrog steps in the Markov transitions of HAIS are sequential and can not be parallelized. See Table~\ref{tab:tab1}.  
Compared with HAIS and AIS, our SteinIS has another advantage: if we want to increase the transitions from 1000 to 2000 for better accuracy, SteinIS can build on the result from 1000 transitions and just need to run another 1000 iterations, while HAIS cannot take advantage of the result from 1000 transitions and have to independently run another 2000 transitions. 

\begin{table}[h]
\label{tab:tab1}
\centering
\caption{Running Time (in seconds) on  MNIST, using the same setting as in Figure~\ref{figdecode}. We use 1000 transitions in all methods to test the running time.}
\vspace{3bp} \begin{tabular}{|c|c|c|c|}
% \begin{centering}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Dimensions of $\bd{z}$ & 10  & 20  & 50  \\ \hline
  SteinIS & 224.40 & 226.17 & 261.76 \\ \hline
  HAIS-10L & 600.15 & 691.86 & 755.44 \\ \hline
  HAIS-1L & 157.76 & 223.30 & 256.23 \\ \hline
  AIS & 146.75 & 206.89 & 230.14 \\
  \hline
% \end{centering}
\end{tabular}
\label{timetable}
\end{table}


==> SteinIS 2/tex/introduction.tex <==
% \section{\normalsize{INTRODUCTION}}
\section{INTRODUCTION}
Probabilistic modeling provides a fundamental framework for reasoning under uncertainty and modeling complex relations in machine learning. % and statistics.
A critical challenge, however, is to develop efficient computational techniques for
approximating complex distributions. Specifically,
given a complex distribution $p(\bd x)$,
often known only up to a normalization constant,
we are interested estimating integral quantities $\E_{p}[f]$  for test functions $f.$
%The most widely used
Popular approximation algorithms
include particle-based methods, such as
Monte Carlo, which construct a set of independent particles $\{\vv x_i\}_{i=1}^n$
%and approximate the expectation using the
whose empirical averaging $\frac{1}{n}\sum_{i=1}^n f(\vv x_i)$
forms unbiased estimates of $\E_p[f]$,
%\E_p f$;
and %optimization-based methods, such as
variational inference (VI),
which approximates $p$ with a simpler surrogate distribution $q$
by minimizing a KL divergence objective function within a predefined parametric family of distributions.
Modern variational inference methods have found successful applications in
highly complex learning systems \citep[e.g., ][]{hoffman2013stochastic, kingma2013auto}. However, VI critically depends on the choice of parametric families and does not generally provide consistent estimators like particle-based methods.
%which may introduce deterministic biases
%Combined with stochastic optimization, VI has been sucessfully applied.
%VI has been found to perform fast approximation, but does introduce
%A general framework is particle-based approximation: finding a set of points (particles) $\{x_i\}_{i=1}^n$ such that $\E_{p} f \approx  \frac{1}{n}\sum_{i=1}^n f(x).$
%construct

%Compl%e
%Approximation of
%Approximate variational inference
Stein variational gradient descent (SVGD) is an alternative
framework that integrates both the particle-based and variational ideas.
% combines the advantages of particle-based methods and variational methods.
%It is based
%particle approximation algorithm motivated by measure transport. % \citep{}\todo{cite optimal}.
It starts with a set of initial particles
$\{\vv x_i^0\}_{i=1}^n$, and
iteratively updates the particles using adaptively constructed {deterministic variable transforms:} %$\T_t$, %at the $t$-th iteration,
%adaptively constructs a deterministic variable transforms $\T_t$, at the $t$-th iteration,
%and and use them to update the particles
$$\bd{x}_i^{\ell} \gets \T_{\ell}(\bd{x}_i^{\ell-1}), ~~~~\forall i= 1,\ldots, n,$$
%where $\ell=1, \ldots, K, $ $K$ is the number of iterations  and
where $\T_\ell$ is a variable transformation at the $\ell$-th iteration that maps old particles to new ones,
% constructed in a nonparametric form. The transform $\T_\ell$
constructed adaptively at each iteration based on the most recent particles $\{\bd{x}_i^{\ell-1}\}_{i=1}^n$
that guarantee to push the particles ``closer'' to the target distribution $p$, in the sense that the KL divergence between the distribution of the particles and the target distribution $p$ can be iteratively decreased.
More details on the construction of $\T_\ell$ can be found in Section 2.
%that
%Here
%It iteratively updates a set of particles %$\{x_i\}_{i=1}^n$ %, where $t$ is the iteration number, with adaptively constructed \emph{deterministic variable transforms} %$\T_t$
%that greedily decrease the KL divergence with the target distribution.
%To be more spe
%Briefly speaking,
%Let $\{x_i^t\}$ be the particles at the $t$-th iteration, SVGD constructs a deterministic transform $\T_t$ which pushes the current particles towards the target distribution
%based on the current parc
%At the $t$-th iteration, SVGD constructs a deterministic transform $\T_t$ based on its current particle $\{x_i^t\}$ that grantesses to push
%push
%$$x_i^{t} \gets \T_{t}(x_i^{t-1}), ~~~~\forall i= 1,\ldots, n,$$
%where $T_t$ is a map, of form $T_t(x) = x + \epsilon \phi(x)$,
%constructed to in order to optimally maximize the KL divergence between the particle distribution and the target distribution.

In the view of measure transport, SVGD iteratively transports the initial probability mass of the particles to the target distribution.
SVGD constructs a path of distributions that bridges the initial distribution $q_0$ to the target distribution $p$,
\begin{align}\label{equ:qt1}
q_{\ell} =  (\T_{\ell} \circ \cdots \circ \T_{1})\sharp q_0, \quad \ell=1, \ldots, K.
\end{align}
where $\T \sharp q$ denotes the push-forward measure of $q$ through the transform $\T$, that is the distribution of $\vv z = \T(\vv x)$ when $\vv x\sim q$.
%Empirically, this process is converges fast because it is deterministic and leverages gradient information of the targtet disstirbution effiiently.

The story, however, is complicated
by the fact that the transform $\T_\ell$ is practically constructed on the fly \emph{depending} on the recent particles $\{\vx_i^{\ell-1}\}_{i=1}^n$,
which introduces complex dependency between the particles at the next iteration,
whose theoretical understanding requires mathematical tools in interacting particle systems \citep[e.g.,][]{braun1977vlasov, spohn2012large, del2013mean} and propagation of chaos \citep[e.g.,][]{sznitman1991topics}.
% \todo{Del Moral book and
% Alain-Sol Sznitman. Topics in propagation of chaos. pages 165?251. Springer, Berlin, 1991.},
As a result, $\{\vv x_i^{\ell}\}_{i=1}^n$ can not be viewed as i.i.d. samples from $q_\ell$.
%which makes it \eqref{equ:qt1}
%However, because the transform $T_t$ is constructed on the fly based on the current particle $\{x_i^{t-1}\}$,
%the particles
%This defines
%As a consequence, this makes the particles independent with each other in a complex fashion, and
This makes it
%conceptually more involved to understand SVGD than the traditional methods such as Monte Carlo,  and
difficult to analyze the results of SVGD and quantify their bias and variance.

In this paper,
we propose a simple modification of SVGD
that ``decouples'' the particle interaction
%R%we propose a simple modification of SVGD that allows us to
and returns particles i.i.d. drawn from $q_\ell$;
we also develop a method to iteratively keep track of the importance weights of these particles,
which makes it possible to give consistent, or unbiased estimators within finite number of iterations of SVGD. %i%n order to correct the bias introduced because of the inconsistency between $\mu_t$ and the target distribution $\mu_p$.

Our method integrates %the advantages
 SVGD with importance sampling (IS) and combines their advantages:
%that is,
it leverages the SVGD dynamics to obtain high quality proposals $q_\ell$ for IS
and also turns SVGD into a standard IS algorithm, inheriting the interpretability and theoretical properties of IS.
%unbiasesss and analysitical results of Monte Carlo that allows us to construct confidence interval for our estimators.
Another advantage of our proposed method is that it
provides an SVGD-based approach for estimating intractable normalization constants,
%which is competitive with  %(or partition function),
%which the original SVGD does not promise.
an inference problem that the original SVGD does not offer to solve.

\paragraph{Related Work}
%
Our method effectively turns SVGD into a nonparametric, adaptive importance sampling (IS) algorithm,
where the importance proposal $q_\ell$ is adaptively improved by the optimal transforms $\T_\ell$ which maximally decreases the KL divergence between the iterative distribution and the target distribution in a function space.
This is in contrast to
the traditional adaptive importance sampling methods
\citep[e.g.,][]{cappe2008adaptive, ryu2014adaptive, cotter2015parallel},
which optimize the proposal distribution from predefined distribution families $\{q_{\bd{\theta}}(\bd{x})\}$, 
%or incorporate IS into parallel MCMC by choosing the importance proposal from mixture families or exponential families.
% indexed by finite numbers of parameters.
often mixture families or exponential families. 
The parametric assumptions restrict the choice of the proposal distributions
and may give poor results when the assumption is inconsistent with
the target distribution $p$.  %deviates from the assumption significantly.
The proposals $q_\ell$ in our method, however, are obtained by recursive variable transforms constructed in a nonparametric fashion
and become more complex as more transforms $\T_\ell$ are applied.
%Because each transform $T_t$, as constructed by SVGD, is highly nonlinear,
%$\mu_t$ can be highly complex when pushed through $T_t$ for a few times.  %recursively.
In fact, one can view $q_\ell$ as the result of pushing $q_0$ through a neural network with $\ell$-layers,
constructed in a non-parametric, layer-by-layer fashion,
which provides a much more flexible distribution family than typical parametric families such as mixtures or exponential families.
%In fact, b
%For example,
% However, when $p(\bd{x})$ is complex and highly skewed from the approximating distribution families they choose, it is difficult to find an appropriate importance proposal from specific distribution families based on traditional adaptive IS aforementioned.
% ~\citet{cappe2008adaptive} apply general mixture families $\{q_{\theta}(\bd{x})\}$
%Monte Carlo methods play a fundamental role in modern Bayesian inference and machine learning. When it is intractable to directly draw samples from the target distribution $p(\bd{z})$ for inference tasks, importance sampling (IS) is one widely used tool to address this problem. IS draws samples $\{\bd{z}_i\}$ from a simpler proposal $q_0(\bd{z})$ and introduces a set of importance weights that are proportional to $p(\bd{z}_i)/q_0(\bd{z}_i),$ which provides an unbiased Monte Carlo estimator. Unfortunately, IS has critical weaknesses which limit their applications. IS heavily depends on the proposal $q_0(\bd{z})$ and is challenging to easily design a good proposal $q_0(\bd{z})$ in high dimensional statistics.
%One approach to address this problem is adaptive IS~\citep{cappe2008adaptive, ryu2014adaptive}, which chooses importance proposals of IS from specific distribution families $\{q_{\theta}(\bd{x})\}$.
% ~\citet{cappe2008adaptive} apply general mixture families $\{q_{\theta}(\bd{x})\}$ as importance proposals for IS and optimize parameters $\theta$ via minimizing the Kullback-Leibler(KL) divergence between $q_{\theta}(\bd{x})$ and $p(\bd{x}).$
 %~\citet{ryu2014adaptive} uses exponential families $\{q_{\theta}(\bd{x})\}$ as importance proposals and  achieves the optimal proposal $q_{\theta^*}(\bd{x})$ by minimizing the variances of interested estimators via stochastic convex programming.
%To overcome the limitation of choosing importance proposal from specific distribution families in traditional adaptive IS, we propose a new adaptive IS, motivated by the iterative transformations for approximating the target distribution defined in \citet{liu2016stein}. We address the problem of finding approximate importance proposals for IS by transforming any initial proposal $q_0(\bd{z_0})$ to our importance proposal $q_K(\bd{z_K})$ through a set of successive transformations, $\bd{z}_K =f_K\circ\cdots\circ f_2 \circ f_1(\bd{z}_0)$. It is easy to obtain a set of samples from $q_K(\bd{z})$ to perform IS via evolving them along these transformations.
%Compared with adaptive IS \citep{cappe2008adaptive, ryu2014adaptive}, our proposed algorithm has two advantages. First, we don't need to restrict our importance proposal to specific distribution families. Instead, our importance proposals can be iteratively transformed from any initial distribution and numerical experiments demonstrate that its $\KL$ divergence with the target distribution can be decreased to be sufficiently small as long as enough successive transformations are performed. Also, our algorithm can be applied to refine the optimal proposal obtained from  \citet{cappe2008adaptive} and \citet{ryu2014adaptive}.  Second, our algorithm can be viewed as nonparametric adaptive IS. The successive transformations we perform optimally decreases the $\KL$ divergence between the proposals and the target distribution in the function space. There is no need to spend extra efforts in optimizing parameters as in traditional adaptive IS.

There has been a collection of recent works %, mostly both in the context of variational inference
 \citep[such as][]{rezende2015variational, kingma2016improved, marzouk2016introduction, spantini2017inference},
%and uncertainty quantification \citep[e.g.,][]{marzouk2016introduction},
that approximate the target distributions
with complex proposals obtained by iterative variable transforms in a similar way to our proposals $q_\ell$ in \eqref{equ:qt1}.
The key difference, however, is that these methods explicitly parameterize the transforms $\T_\ell$
and optimize the parameters by back-propagation,
while our method, by leveraging the nonparametric nature of SVGD,
constructs the transforms $\T_\ell$ sequentially in closed forms,
requiring no back-propagation.
%constructs the transforms sequentially,
%with a predefined layer.
%$whose optimizatin is often complex because it involve
%Recently,  in variational inference, \citet{liu2016stein}, \citet{rezende2015variational}, and \citet{marzouk2016introduction} propose to use a set of sequential transformations to transform any initial distribution $q_0(\bd{z_0})$ into the inference distribution $q_K(\bd{z_K})$ which arbitrarily approximates the target distribution $p(\bd{z})$. Their variational algorithms overcome the limitation of employing simple families of posterior approximations(mean-filed or other simple structured approximations). ~\citet{rezende2015variational} and ~\citet{marzouk2016introduction} first parameterizes the transformations and optimize these parameters via amortized variational inference. While \citet{liu2016stein} first derive optimal transformations using a functional gradient descent which minimizes the $\KL$ divergence between $q_K(\bd{z})$ and $p(\bd{z})$ without explicit parametric assumptions and then approximates these transformations by evolving a set of particles.
%Compared with the original version of SVGD, our main advertage is that it is a typical adaptive Monte Carlo

%Although the transformations we define have the same form in Stein variational gradient descent(SVGD) \citep{liu2016stein}, there are three main differences between our algorithm and SVGD. First, we have different purposes on applications. SVGD runs a set of particles to approximate the target distribution.  Our algorithm keeps track of the sequential distributions to approximate a target distribution.   Second, the particles from SVGD are interactive and dependent with each other. Unless sufficient iterations are implemented in SVGD, the estimations provided by SVGD are biased. Inheriting the unbiased property of IS, our method can provide unbiased estimation at every iteration. And the particles evolved in our algorithms are independent from each other. Finally, since we know the distribution of our particles, we can examine the KL divergence between the successive distributions we evolve and the target distributions. Our algorithm can be applied to more general inference tasks such as estimating the partition functions in graphical models and evaluating $\log $ likelihoods of generative models while SVGD cannot be.

The idea of constructing a path of distributions $\{q_\ell\}$ to bridge
the target distribution $p$ with a simpler distribution $q_0$
invites connection to ideas such as annealed importance sampling (AIS) \citep{neal2001annealed}
and path sampling (PS) \citep{gelman1998simulating}.  % \todo{ADD citation: Simulating normalizing constants: from importance sampling to bridge sampling to path sampling}.
These methods typically construct an annealing path using geometric averaging of the initial and target densities instead of variable transforms,
which does not build in a notion of variational optimization as the SVGD path.
In addition, it is often intractable to directly sample distributions on the geometry averaging path,
and hence  AIS and PS  need additional mechanisms in order to construct proper estimators.
% the distributions on the
%and
%which does not adaptively minimizes KL divergence as $q_t$ and
%and does not adaptively
%which may not have the nice properties as ours.
%In addition, these methods work in different ways: our method is a standard adaptive importance sampling with proposal $\mu_t$,which AIS and PS  need additional mechainisms because $\mu_t$ construct from geometric averaging is not directly intractable to draw samples, and additional mechisimas are needed in order to constuct proper estimators.
%There are two key differences, first, our method is a standard importance
%is similar to
%It is interesting to note that our algorithm that iteratively transforms the initial distribution $q_0(\bd{z})$ to the importance proposal $q_K(\bd{z})$ is contrastive to annealing importance sampling(AIS)~\citep{neal2001annealed} which constructs the annealing path to connect $p(\bd{z})$ with $q_0(\bd{z})$ for implementing IS through a chain of Markov transitions, usually by geometric averages of the initial proposal $q_0(\bd{z})$ and the target $p(\bd{z})$.

% \todo{adjust outline}
{\bf Outlines} The reminder of this paper is organized as follows. 
Section 2 discusses Stein discrepancy and SVGD. 
We propose our main algorithm in Section 3, and a related method in Section 4. %introduces a new algorithm. 
Section 5 provides empirical experiments and Section 6 concludes the paper. 


==> SteinIS 2/tex/mainmethod.tex <==
% \section{\normalsize{DECOUPLING SVGD}}%Turning it into Importance Sampling}
\section{DECOUPLING SVGD}
In this section, we introduce our main Stein variational importance sampling~(SteinIS) algorithm. Our idea is simple.
We initialize the particles $\{\vx_i^0\}_{i=1}^n$ by i.i.d. draws from an initial distribution $q_0$ and partition them into two sets,
including a set of \emph{leader particles} $\vx_A^\ell = \{\vx_i^\ell  \colon  i\in A\}$
and
 \emph{follower particles}
$\vx_B^\ell = \{\vx_i^\ell  \colon  i\in B\}$, with $B =  \{1,\ldots, n\} \setminus A$,
where the leader particles $\vx_A^\ell$ are responsible for constructing the transforms, using the standard SVGD update \eqref{equ:svgdup2},
%is updated by SVGD dynamics \eqref{equ:svgdup2} as before,
%which simultaneously pushed by map $\T_t$ and contributes to the construction of the next map $\T_{t+1}$,
while the follower particles $\vx_B^\ell$ simply follow the transform maps constructed by $\vx_A^\ell$ and do not contribute to the construction of the transforms. 
In this way, the follower particles $\vx_B^{\ell}$ are independent conditional on the leader particles $\vx_A^\ell$. 
%$\T_{t+1}$.

Conceptually, we can think that we first construct all the maps $\T_\ell$ by evolving the leader particles $\vx_A^\ell$,
and then push the follower particles through $\T_\ell$ in order to draw exact, i.i.d. samples from $q_\ell$ in \eqref{equ:qt}.
Note that this is under the assumption the leader particles $\vx_A^\ell$
has been observed and fixed, which is necessary because the transform $\T_\ell$ and
distribution $q_\ell$ depend on $\vx_A^\ell$.
% \vspace{-0.4cm}
\begin{figure}[tbp]
   \centering
 \includegraphics[width=.32\textwidth]{figures/leader.pdf} % requires the graphicx package
  % \includegraphics[width=.3\textwidth]{figures/leader}
   \vspace{-.45\baselineskip}
   \caption{\small
   %Illustrating of our method.
   Our method uses a set of leader particles $\vx_A^\ell$ (green) to construct the transform map $\T_\ell$,
   which follower particles $\vx_B^\ell$ follows subsequently. The leader particles $\vx_A^\ell$ are interactive and dependent on each other.
   The follower particles $\vx_B^\ell$ can be viewed as i.i.d. draws from $q_\ell$, given fixed leader particles $\vx_A^\ell$.
   }
   \label{fig:example}
\end{figure}

In practice, however, we can simultaneously update both the leader and follower particles, by a simple modification of the original SVGD \eqref{equ:svgdup2} shown in Algorithm~\ref{VarIS:algo} (step 1-2),
where the only difference is that we restrict the empirical averaging in \eqref{equ:phit} to the set of % is restricted on
the leader particles $\vx_A^\ell$. The relationship between the particles in set $A$ and $B$ can be more easily understood in Figure~\ref{fig:example}.
\begin{algorithm}[tb] %
\caption{Stein Variational Importance Sampling}  \label{VarIS:algo}
\begin{algorithmic}
\STATE {\bf Goal}: Obtain i.i.d. importance sample $\{\vx_i^K, ~ w_i^K\}$ for $p$.
\STATE {Initialize} $\vx_{A}^0$ and $\vx_B^0$ by i.i.d. draws from $q_0$.
\STATE {Calculate} $\{ q_0(\vx_i^0) \}, \forall i\in B.$
%Initialize particles $\{\vv z_{i}\}^N$i.i.d. from $q_0$. Take a subset $A$ of particles as the leaders and the remaining $B = [N]\setminus A$ as the followers.
%$\vv z_{L}^0$ and follower particles $\vv z_{F}^0$.
\FOR{iteration $\ell =0, \ldots, K-1$}
\STATE
%\vspace{-1\baselineskip}
%\!\!\!
1. Construct the map using the leader particles $\vx_A^\ell$%5 both the leader and follower particles %in $A \cup B$ by
\begin{align}\notag%\label{equ:ffa}
%\!\!\!\! \!\!\!\!  \!\!\!\!  \!\!\!\!
 \!\!\!\! \!\!\!\!
\ff_{\ell+1}(\cdot) =  \frac{1}{|A|}\sum_{j\in A} [\nabla \log p(\vv x_j^\ell) k(\vv x_j^\ell,  \cdot) + \nabla_{\vv x_j^\ell} k(\vv x_j^\ell, \cdot)].
\end{align}
%\!\!\!\!\!\!\!\!\!\!\!\!\!\!T_{t+1}(\vv x) =  \vv x + \epsilon\frac{1}{|A|}\sum_{j\in A} [\nabla \log p(\vv z_j) k(\vv z_j,  \vv x) + \nabla_{\vv z_j^t} k(\vv z_j^t, \vv x)].
2. Update both the leader and follower particles %in $A \cup B$ by
$$
%\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\vv x_{i}^{\ell+1} \gets \vv x_i^\ell + \epsilon \ff_{\ell+1}(\vv x_i^\ell), ~~~~ \forall i \in A\cup B.
%\vv z_i^t + \epsilon\frac{1}{|A|}\sum_{j\in A} [\nabla \log p(\vv z_j^t) k(\vv z_j^t,  \vv z_i^t) + \nabla_{\vv z_j^t} k(\vv z_j^t, \vv z_i^t)].
$$
3. Update the density values (for $i\in B$) by
\begin{equation*}
q_{\ell+1}(\vx_{i}^{\ell+1}) =  q_{\ell}(\vx_{i}^{\ell}) \cdot  | \mathrm{det}(I ~+~ \epsilon \nabla_{\bd{x}} \bd{\ff}_{\ell+1}(\bd{x}^{\ell}_i))|^{-1}
\end{equation*}
\ENDFOR
\STATE {Calcuate} $w_i^{K} = p(\vv x_i^{K}) / q_K(\vv x_i^{K}), \forall i\in B.$
\STATE {\bf Outputs}: i.i.d. importance sample $\{\vx_i^K, ~ w_i^K\}$ for $i\in B.$
\end{algorithmic}
\end{algorithm}
%\begin{figure}[h]
%\centering
%\begin{tabular}{c}
%\includegraphics[height=0.27\textwidth]{figures/svgd9.pdf}
%\end{tabular}
%\caption{Illustration of Algrithm~\ref{VarIS:algo}. The particles at $\ell$-th iteration in set $A$ are applied to construct the approximate transforms $\{\T_\ell\}$, which is applied to perform transformations for particles in both $A$ and $B$. Since the transforms depends on all particles in $A,$ the updated particles in $A$ via $\{\T_\ell\}$ will depend on each other. While each updated particle in $B$, only depending on $A$, is independent of all other particles in $B.$}
%\label{decouplesvgd}
%\end{figure}

%This can be easily implemented by modifying the original SVGD, such that the empirical averaging in \eqref{equ:phit} is restricted on
%t%he leader particles $\vx_A^t$. See Algorithm~\ref{VarIS:algo}.
%$\sum_{i=1}^n$

%With this simple modification, the follower particles $\vx_B^t$ are coupled with each other only through the leader particles $\vx_A^t$ as visualized in Figure~\ref{graph}, and hence are conditionally independent given fixed observing fixed leader particles $\vx_A^t$.  In addition, $\vx_B^t$ can be viewed as i.i.d. draws from $q_t$, conditioning on fixed $\vx_A^t$.
%if $\{y_i^0\}$ is i.i.d. drawn from $q_0$,
%$\{y_i^{t}\}$ would
%keep independent with each other, and
%$\vx_B^t$ is i.i.d. drawn from $q_t$,
%llows
%This is
%the trajectory of $\{x_i\}$.
%a set of p
%In order to generate i.i.d. sample from $q_t$,
%We introduce an additional set of particles $\{y_i\}$ in additional to the $\{x_i\}$ updated by
%\eqref{equ:svgdup2}, where ${x_i}$ is responsible for constructing $\T_t$ and $q_t$, while ${y_i}$ simply follows the updates constructed by $\{x_i\}$
%and do not influence the trajectory of $\{x_i\}$,
%that is,
%$$
%y_{i}^{t+1} \gets \T_{t+1}(y_{i}^t),
%$$
%where $\T_{t+1}$ is constructed based on $x_i^t$ in \eqref{equ:phit} and \eqref{equ:svgdup2}, and does not depend on $\{y_i^{t}\}.$
%In this way,
%if $\{y_i^0\}$ is i.i.d. drawn from $q_0$,
%$\{y_i^{t}\}$ would
%keep independent with each other, and exactly draws from $q_t$, conditioning on fixed $\{x_i\}$.
%Rcan be viewed as
%whose importance weights wi = p(xi)/ql(xi) can be also calculated efficiently with an iterative update.
%more straightforward methods such as Monte Carlo
%
%In practice, $\{y_i\}$ can be sequentially constructed together with $\{x_i\}$ as shown in Algorithm~\ref{VarIS:algo}. This is a simple modification of SVGD, which simply restricts the empirical summation in $\phi_{t}$ to the set of leader particles. %$\{x_i^{t-1}\}$.


\paragraph{Calculating the Importance Weights}
%
%
%
Because $q_\ell$ is still different from $p$ when we only apply finite number of iterations $\ell$, which introduces deterministic biases if we directly use $\vx_B^\ell$ to approximate $p$.
%in order to get consistent estimation
%it is beneficial to keep track of the importance weights $p(\vx) / q_t(\vx)$ of
%$\vx_B^t$
%it introduces deterministic biases when we directly use $\{y_i^t\}$ to
%approximate $p$.
We address this problem by further turning the algorithm into an importance sampling algorithm with importance proposal $q_\ell$. Specifically, we calculate the importance weights of the particles $
\{\vx_i^\ell\}$:
\begin{align}\label{equ:wt}
w_i^\ell= \frac{\bar p(\vx_i^{\ell})}{q_\ell(\vx_i^\ell)},
\end{align}
where $\bar p$ is the unnormalized density of $p$, that is, $p(\vx) = \bar p(\vx)/Z$ as in \eqref{barp}. 
In addition, the importance weights in \eqref{equ:wt} can be calculated based on the following formula:
\begin{equation}
\label{density}
q_\ell(\bd{x}^\ell)=q_0(\bd{x}^0)\prod_{\jmath=1}^\ell |\mathrm{det}(\nabla_{\bd{x}} \bd{T}_\jmath(\bd{x}^{\jmath-1}))|^{-1},
\end{equation}
where $\bd{T}_\ell$ is defined in~\eqref{equ:svgdup2} and we assume that
 the step size $\epsilon$ is small enough so that each $\T_\ell$ is an one-to-one map.
 As shown in Algorithm~\ref{VarIS:algo} (step 3), 
 \eqref{density} can be calculated recursively as we update the particles. 

With the importance weights calculated, we turn SVGD into a standard importance sampling algorithm. 
For example, we can now estimate expectations of form $\E_p f$ by 
$$
 \hat \E_{p}[f] = \frac{\sum_{i\in B} w_i^\ell f(\vx_i^\ell)}{\sum_{i\in B} w_i^\ell}, 
$$
which provides a consistent estimator of $\E_{p} f$ when we use finite number $\ell$ of transformations.  
Here we use the self normalized weights because
$\bar p(\vx)$ is unnormalized.
Further, the sum of the unnormalized weights provides an unbiased estimation for the normalization constant $Z$:
$$
\hat Z = \frac{1}{|B|} \sum_{i\in B} w_i^\ell,
$$
which satisfies the unbiasedness property $\E[\hat Z] = Z$. Note that the original SVGD does not provide a method for estimating normalization constants,
although, as a side result of this work, Section 4 will discuss another method for estimating $Z$ that is more directly motivated by SVGD.
% known only up to the normalization constant.
%$ to eliminate the deterministic bias.
%$To be specific, we calculate the importance

%It would be nice to keep track of the importance weights $p(\vv y_i) /q_t (\vv y_i)$ in order to perform gradient descent.
%For this purpose, we assume the initial distribution $q_0$ is simple enough so that we can calculate the importance weights $p(\vv y_i^0) /q_0(\vv y_i^0).$

%In order to implement this idea, we need to
%Further, as we update the particles, their corresponding importance weights
%$p(\vv y_i^t) /q_0(\vv y_i^t)$ can be updated iteratively.

We now analyze the time complexity of our algorithm. 
Let $\alpha(d)$ be the cost of computing $\bd{s}_p(\bd{x})$ and 
$\beta(d)$ be the cost of evaluating kernel $k(\vx, \vx')$ and its gradient $\nabla k(\vx, \vx')$. Typically, both $\alpha(d)$ and $\beta(d)$ grow linearly with the dimension $d. $ In most cases, $\alpha(d)$ is much larger than $\beta(d)$. 
The complexity of the original SVGD with $|A|$ particles is $O(|A|\alpha(d)+|A|^2\beta(d))$, 
and the complexity of Algorithm~\ref{VarIS:algo} is $O(|A|\alpha(d)+|A|^2\beta(d)+|B||A|\beta(d)+|B| d^3 ),$   
% \blue{The key computational cost here is to calculate the determinant of the Jacobian matrix, for which typica
%The computational cost of calculating determinants of Jacobian matrices for typical methods is $O(d^3),$  
%So the complexity of Algorithm~\ref{VarIS:algo} is $O(|A|\alpha(d)+|A|^2\beta(d)+|B||A|\beta(d)+|B| d^3 ).$
% \blue{The key computational cost here is to calculate the determinant of the Jacobian matrix, for which typical methods would cost $O(d^3)$ where $d$ is the dimension of $\vx$.
% The total cost of each iteration of Algorithm~\ref{VarIS:algo} is $O(|A| + |B| d^3)$.}
where the $O(|B|d^3)$ complexity comes from calculating the determinant of the Jacobian matrix, 
which is expensive when dimension $d$ is high, but is the cost to pay for having a consistent importance sampling estimator in finite iterations
and for being able to estimate the normalization constant $Z$.
Also, by calculating the effective sample size based on the importance weights, 
we can assess the accuracy of the estimator, and early stop the algorithm when a confidence threshold is reached. 
%The calculation of the importance weights also provides an assessment of accuracy using the effective sample size of the weights and enables us to early stop the algorithm when a confidence threshold is reached.
%and being able to estimation the normalization

One way to speed up our algorithm in empirical experiments is to parallelize the computation of Jacobian matrices for all follower particles in GPU. It is possible, however, to develop efficient approximation for the determinants by leveraging the special structure of the Jacobean matrix; note that %given by
%which may destroys the consistency
%which is given by
% The Jacobian matrix is given by
\begin{align}
&\nabla_{\bd{y}} \bd{T}(\bd{y}) = I  + \epsilon A,  \notag \\
&A = \frac{1}{n}\sum_{j=1}^n [\nabla_{\vv x} \log p(\vv x_j)^\top \nabla_{\vv y} k(\vv x_j, \vv y) +
\nabla_{\vv x} \nabla_{\vv y} k(\vv x_j, \vv y)]. \notag
 \end{align}
 Therefore, $\nabla_{\bd{y}} \bd{T}(\bd{y})$ 
 is close to the identity matrix $I$ when the step size is small.
This allows us to use Taylor expansion for approximation:
 % The computational cost,
%See Algorithm for the update.
%This involve calculating the determinant of $\nabla T$
%We also point out that one drawback of our method is that the determinants of the Jacobians $\{\nabla_{\bd{y}} \hat{\bd{T}}_l\}$ have to be calculated at each iteration. When our algorithm is parallelized in GPU, we find the time spent in each iteration of our algorithm is comparable to the time spent in each Markov transition in annealing importance sampling(AIS). The total time cost spent in our algorithm is comparable with that of Hamiltonian AIS when the same number of transitions are performed on both algorithms. Taking advantage of the special form of Jacobian matrices in our algorithm, the computation of determinants can be speed up when some mild approximation is introduced. Let us denote $\nabla_{\bd{y}} \hat{\bd{T}}_l(\bd{y}) = \bd{I} + \epsilon A , $ where $A=(a_{ij})_{d\times d}$ and $d$ is the dimension of the feature space.
\begin{pro}
\label{detapprox}
%Let $\lambda_k(A)$ be the eigenvalue of $A,$ and $\rho(A)=\max_k|\lambda_k(A)|$ the spectral radius of $A$.
Assume $\epsilon < 1/\rho(A)$, where $\rho(A)$ is the spectral radius of $A$, that is,
 $\rho(A) =\max_j |\lambda_j(A)|$ and $\{\lambda_j\}$ are the eigenvalues of $A$. We have
%and there are some constant $C$ such that $\|A\|_{\infty}\le C,$  then we have
\begin{equation}
\label{Jacobapprox}
\mathrm{det}(I +\epsilon A) =\prod_{k=1}^d (1+\epsilon a_{kk})+ O(\epsilon^2),
\end{equation}
where $\{a_{kk}\}$ are the diagonal elements of $A$.
\end{pro}

\begin{proof}
Use the Taylor expansion of $\mathrm{det}(I +\epsilon A)$. 
%Note that $\mathrm{det}(I +\epsilon A)=\exp(\mathrm{trace}(\log (I +\epsilon A))),$
%and $\log (I +\epsilon A)=1 + \epsilon A + O(\epsilon^2).$ %\sum_{n=1}^\infty \frac{(-1)^{n-1}}{n}\epsilon^nA^n,$
%and $\log (I +\epsilon A)=\sum_{n=1}^\infty \frac{(-1)^{n-1}}{n}\epsilon^nA^n,$
%where $A^n= A^{n-1}A.
%$ T $\mathrm{det}(I +\epsilon A) =\prod_k^d (1+\epsilon a_{kk})+ O(\epsilon^2).$
\end{proof}
Therefore, one can approximate the determinant with approximation error $O(\epsilon^2)$ using linear time $O(d)$ w.r.t. the dimension.
Often the step size is decreasing with iterations,
and a way to trade-off the accuracy with computational cost is to % practical trick is that we can use the exact
use the exact calculation in the beginning when the step size is large,
and switch to the approximation when the step size is small.
%Theorem \ref{detapprox} indicates that when $\epsilon$ is infinitesimal, the determinants of the Jacobian matrices can be approximated by equation \eqref{Jacobapprox} and the approximation error is $O(\epsilon^2).$ In this case, the calculation of these determinants can be implemented in linear time with respect to the feature dimension, i.e., $O(d),$ which helps us speed up our algorithm \ref{VarIS:algo}.
%Therefore,
%we have
%$$
%w_i^{t} = \frac{}{}
%$$
%we ha
%we can calculate
%In order to calculate the
%
%
%Before introducing our nonparametric variational adaptive importance sampling, let us first illustrate the idea of invertible transformations of random variables. Suppose the density function of random variable $\bd{x}$ is $q(\bd{x})$ and the invertible transformation is $\bd{z}=\bd{T}(\bd{x}),$ then the density function of $\bd{z}$ is $$q_{[\bd{T}]}(\bd{z})=q(\bd{x})|\mathrm{det}(\nabla_{\bd{z}} \bd{T}^{-1}(\bd{z}))|=q(\bd{x})|\mathrm{det}(\nabla_{\bd{x}} \bd{T}(\bd{x}))|^{-1}.$$

%If we apply the invertible mapping sequentially, $$\bd{z}^j=\bd{T}_j\circ\cdots\bd{T}_2\circ \bd{T}_1(\bd{z}^0),$$ for $j=1, 2,\cdots, K,$
%then the density function of $z_K$ satisfies,
%\begin{equation}
%\label{density}
%q_K(\bd{z}^K)=q_0(\bd{z}^0)\prod_{j=1}^K |\mathrm{det}(\nabla_{\bd{z}} \bd{T}_j(\bd{z}^{j-1}))|^{-1},
%\end{equation}
%where the density function of random variable $\bd{z}^0$ is $q_0.$
%Taking advantage of the simple transformations defined in SVGD, we construct our sequential transformations as follows,
%\begin{equation}
%\label{transform}
%\bd{z}^{j+1} =\bd{T}_{j+1}(\bd{z}^{j})=\bd{z}^{j}+\epsilon \bd{\phi}_{j}(\bd{z}^{j}),
%\end{equation}
%where based on equation \eqref{transf}, $\phi_j(\cdot)$ is defined as follows,
%\begin{equation}
%\label{stein}
%\phi_j(\cdot)=\mathbb{E}_{\bd{z}\sim{q_j}}[\nabla_{\bd{z}} \log p(\bd{z})k(\bd{z},\cdot)+\nabla_{\bd{z}} k(\bd{z},\cdot)],
%\end{equation}
%for $j=0, 1, 2,\cdots K-1$.
%Empirically, starting from  a set of samples $\{\bd{z}_i^0\}_{i=0}^N$ drawn from $q_0(\bd{z}^0),$ the simple transformation (\ref{transform}) can be approximated by
%\begin{equation}
%\label{approxtransf}
%\hat{\bd{T}}_j(\bd{x})=\bd{x}+\frac{\epsilon}{N}\sum_{i=1}^N[\nabla_{\bd{z}} \log p({\bd{z}}^{j}_i)k(\bd{z}^j_i,\bd{x})+\nabla_{\bd{z}} k(\bd{z}^j_i,\bd{x})],
%\end{equation}
% and hence $\bd{z}^j_i=\hat{\bd{T}}_j(\bd{z}_i^{j-1})$ for $i=1, 2, \cdots, N.$ We observe that particles $\{\bd{z}^j_i\}$ transformed from $\hat{\bd{T}}_j$ are interactive and dependent on each other. As we approximate the transformations,  we can draw another set of $\{\bd{y}_i^0\}_{i=0}^M$ and apply the sequential transformations $\{\hat{\bd{T}}_j\}$ to this set of particles simultaneously. Note that different from $\{\bd{z}^j_i\}_{i=1}^N,$ samples $\{\bd{y}^j_i\}_{i=1}^M$ are independent, for $j=1,2,\cdots, K$. Based on equation \eqref{density}, we can empirically approximate the densities of particles $\{\bd{y}^K_i\}_{i=1}^M$ as follows,
%\begin{equation}
%\label{approxden}
%\hat{q}_K(\bd{y}^K_i)=q_0(\bd{y}^0_i)\prod_{j=1}^K |\mathrm{det}(\nabla_{\bd{y}} \hat{\bd{T}}_j(\bd{y}^{j-1}_i))|^{-1},
%\end{equation}
%for $i=1, 2, \cdots, M.$ These independent particles $\{\bd{y}^K_i\}_{i=1}^M$ along with their density values $\{\hat{q}_K(\bd{y}^K_i)\}_{i=1}^M$ can be employed to implement importance sampling, which is summarized in Algorithm \ref{VarIS:algo}.
%
%
%
%\begin{algorithm*}[tb]
%\caption{Stein Variational Adaptive Importance Sampling(SteinIS)}
%\label{VarIS:algo}
%\begin{algorithmic}[1]
%\STATE {\bfseries Input:} Two sets of particles $\{\bd{z}_i^0\}_{i=1}^N\sim q_0(\bd{z})$ and $\{\bd{y}_i^0\}_{i=1}^M\sim q_0(\bd{y}).$
%\STATE {\bfseries Output:} A set of particles $\{\bd{y}_i^K\}$ with importance weights $\{\hat{q}_K(\bd{y}^K_i)/p(\bd{y}^K_i)\}.$
%denote $H(\theta,\eta) = -\nabla_{[\theta,\eta]}^2 \log p({\theta},{\eta}|{X})$; budget size $\mk$.
%\FOR{$j=1,2,\cdots,K$}
%\STATE{Calculate $\bd{z}^j_i=\hat{\bd{T}}_j(\bd{z}^{j-1}_i)$ for $i=1,2,\cdots N$ via equation (\ref{approxtransf}).}
%\STATE{Compute $\bd{y}^j_i=\hat{\bd{T}}_j(\bd{y}^{j-1}_i)$ and $\mathrm{det}(\nabla_{\bd{y}}\hat{\bd{T}}_j(\bd{y}^{j-1}_i))$ via equation (\ref{approxtransf}) for $i=1,2,\cdots M.$}
%\ENDFOR
%\STATE{Calculate importance weights $\{\hat{q}_K(\bd{y}^K_i)/p(\bd{y}^K_i)\}$ via equation (\ref{approxden}).}
%the following M-estimator, $$\boldsymbol{\hat{\theta}}_{\KL-W}=\argmax_{\boldsymbol{\theta}\in\Theta}\sum_{k=1}^d\frac1n\sum_{j=1}^n\frac{p(\boldsymbol{\widetilde{x}}_j^k| \boldsymbol{\hat{\theta}}_k)}{p(\boldsymbol{\widetilde{x}}_j^k| \boldsymbol{\widetilde{\theta}}_k)}\log p(\boldsymbol{\widetilde{x}}_j^k| \boldsymbol{\theta}).$$
%\end{algorithmic}
%\end{algorithm*}

 %We emphasize that Algorithm \ref{VarIS:algo} is different from SVGD on two aspects. First, SVGD only iteratively evolves interacting particles $\{\bd{z}^j_i\}_{i=1}^N$ which are dependent with each other. While our SteinIS uses another set of independent particles $\{\bd{y}^j_i\}_{i=1}^M.$ As we will prove later, the empirical probability measure of $\{\bd{y}^K_i\}_{i=1}^M$ will converge to the exact probability measure with density function $q_K$ in some measure metric when $N\to \infty$ and $M\to \infty$.
% Second, our algorithm calculates the determinants of Jacobian matrices of successive transformations so that we know the approximate density values of the particles $\{\bd{y}^j_i\}_{i=1}^M.$ There are two advantages of computing the determinants although it increases the computational cost at each iteration.
% One is that inheriting from the unbiased property of IS, our algorithm can provide unbiased estimation when we stop at early iteration. SVGD provides biased estimations for inference tasks unless sufficient iterations are performed to ensure the evolved particles have converged. Another advantage is that our algorithm enables us to do more inference tasks on which SVGD cannot be applied such as estimating the partition functions of unnormalized distributions.

% We also point out that one drawback of our method is that the determinants of the Jacobians $\{\nabla_{\bd{y}} \hat{\bd{T}}_l\}$ have to be calculated at each iteration.

%\red{check, todo}
%The speed of Algorithm 1 can be further improved by efficient GPU implementation.
% When our algorithm is parallelized in GPU \todo{paralleize which part?},
% we find the time spent in each iteration of our algorithm  (with the exact determinant computation) is comparable to the time spent in each Markov transition in annealing importance sampling(AIS) with dimension XXX and comparable particle sizes???.
%The total time cost spent in our algorithm is comparable with that of Hamiltonian AIS \citet{cite}
%  when the same number of transitions are performed on both algorithms.

%  Taking advantage of the special form of Jacobian matrices in our algorithm, the computation of determinants can be speed up when some mild approximation is introduced. Let us denote $\nabla_{\bd{y}} \hat{\bd{T}}_l(\bd{y}) = \bd{I} + \epsilon A , $ where $A=(a_{ij})_{d\times d}$ and $d$ is the dimension of the feature space.
%\begin{thm}
%\label{detapprox}
%Let $\lambda_k(A)$ be the eigenvalue of $A,$ the spectral radius $\rho(A)=\max_k|\lambda_k(A)|$, $\epsilon$ is chosen such that $\epsilon\rho(A)<1$ and there are some constant $C$ such that $\|A\|_{\infty}\le C,$  then we have
%\begin{equation}
%\label{Jacobapprox}
%\mathrm{det}(I +\epsilon A) =\prod_{k=1}^d (1+\epsilon a_{kk})+ O(\epsilon^2).
%\end{equation}
%\end{thm}
%{%\bf Proof:} we know $\mathrm{det}(I +\epsilon A)=\exp(\mathrm{trace}(\log (I +\epsilon A))),$ $\log (I +\epsilon A)=\sum_{n=1}^\infty \frac{(-1)^{n-1}}{n}\epsilon^nA^n,$
%where $A^n= A^{n-1}A.$ Therefore, we have $\mathrm{det}(I +\epsilon A) =\prod_k^d (1+\epsilon a_{kk})+ O(\epsilon^2).$ \\

%Theorem \ref{detapprox} indicates that when $\epsilon$ is infinitesimal, the determinants of the Jacobian matrices can be approximated by equation \eqref{Jacobapprox} and the approximation error is $O(\epsilon^2).$ In this case, the calculation of these determinants can be implemented in linear time with respect to the feature dimension, i.e., $O(d),$ which helps us speed up our algorithm \ref{VarIS:algo}.
%  \subsection{MONTONE DECREASING OF THE KL DIVERGENCE}
% \subsection{\normalsize{MONTONE DECREASING OF THE KL DIVERGENCE}}
\subsection{Monotone Decreasing of KL divergence} % between $q_\ell$ and $p$}
One nice property of algorithm~\ref{VarIS:algo} is that the KL divergence between the iterative distribution $q_\ell$ and $p$ is monotonically decreasing. This property can be more easily understood by considering our iterative system in continuous evolution time as shown in \citet{liu2017stein}. 
Take the step size $\epsilon$ of the transformation defined in \eqref{update} to be infinitesimal, 
and define the continuos time $t = \epsilon \ell$. Then the evolution equation of random variable $\vx^t$ is governed by the following nonlinear partial differential equation~(PDE), 
\begin{equation}
\label{part}
\frac{d\bd{x}^t}{dt}=\mathbb{E}_{\bd{x}\sim{q_t}}[\bd{s}_p(\bd{x})k(\bd{x},\bd{x}^t)+\nabla_{\bd{x}} k(\bd{x},\bd{x}^t)],
\end{equation}
where $t$ is the current evolution time and $q_t$ is the density function of $\vx^t.$ The current evolution time $t= \epsilon \ell$ when $\epsilon$ is small and $\ell$ is the current iteration. We have the following proposition (see also \citet{liu2017stein}): 
\begin{pro}
\label{pro2}
Suppose random variable $\bd{x}^t$ is governed by PDE \eqref{part}, then its density $q_t$ is characterized by
\begin{equation}
\label{diffode}
\frac{\partial q_t}{\partial t}=-\mathrm{div}(q_t\mathbb{E}_{\bd{x}\sim{q_t}}[\bd{s}_p(\bd{x}) k(\bd{x},\bd{x}^t)+\nabla_{\bd{x}} k(\bd{x},\bd{x}^t)]),
\end{equation}
where $\mathrm{div}(\bd{f})=\trace(\nabla \vv f) = \sum_{i=0}^d \partial f_i(\bd{x})/\partial x_i$, and  $\bd{f}=[f_1,\ldots, f_d]^\top.$ %$\mathrm{div}\boldsymbol{f}(x)=\sum_{i=1}^d\frac{\partial f_i}{\partial x_i}.$
\end{pro}
The proof of proposition~\ref{pro2} is similar to the proofs of proposition 1.1 in~\citet{jourdain1998propagation}. 
%and lemma 3 in ~\citet{dai2016opaque}. 
Proposition~\ref{pro2} characterizes the evolution of the density function $q_t(\bd{x}^t)$ when the random variable $\bd{x}^t$ is evolved by ~\eqref{part}. The continuous system captured by~\eqref{part} and ~\eqref{diffode} is a type of Vlasov process which has wide applications in physics, biology and many other areas~\citep[e.g.,][]{braun1977vlasov}.
As a consequence of proposition~\ref{pro2}, one can show the following nice property:
\begin{equation}
\label{klksd}
\frac{d\mathrm{KL}(q_t\mid\mid p)}{dt}=-\mathbb{D}(q_t ~||~ p)^2<0,
\end{equation}
which is proved by theorem 4.4 in \citet{liu2017stein}. 
Equation ~\eqref{klksd} indicates that the KL divergence between the iterative distribution $q_t$ and $p$ is monotonically decreasing with a rate of $\mathbb{D}(q_t~||~ p)^2$. 

\iffalse
% \subsection{Theoretical Investigation of SteinIS}
\subsection{\normalsize{THEORETICAL INVESTIGATION OF STEINIS}}
In this section, we provide some theoretical investigation of our proposed algorithm. The analysis of our algorithm is based on the theoretical results of SVGD. First, we establish the convergence property of our algorithm w.r.t. the number of particles. Then, we provide some analysis on the convergence rate of our importance proposal $q_K$ to the target distribution $p$.

The convergence rate w.r.t. the particles size can be more easily illustrated in terms of the empirical measures induced by the evolved particles $\{\bd{z}^j_i\}_{i=1}^N$ and $\{\bd{y}^j_i\}_{i=1}^M$. The empirical measures of these two sets of particles are defined as
\begin{equation*}
\begin{split}
&\widetilde{\mu}^j_N(d\bd{x})=\frac1N\sum_{i=1}^N\delta(\bd{x}-\bd{z}^j_i)d\bd{x},\\
& \hat{\mu}^j_M(d\bd{x})=\frac{1}{M}\sum_{i=1}^M\delta(\bd{x}-\bd{y}^j_i)d\bd{x},
\end{split}
\end{equation*}
where $\delta$ is the dirac function. Denote $\mu_{\infty}^j$ as the exact probability measure with density function $q_j$, which is the density of $\bd{z}^j$ defined by equation \eqref{transform} and \eqref{stein}. We define the bounded Lipschitz of function $f$ as
\begin{equation*}
\|f\|_{\mathrm{BL}}= \max\{\sup_{\bd{x}}|f(\bd{x})|, \sup_{\bd{x}\neq \bd{y}} \frac{|f(\bd{x})-f(\bd{y})|}{\|\bd{x}-\bd{y}\|_2}\}.
\end{equation*}
For vector-valued $\bd{f}=[f_1,\cdots, f_d],$ $\|\bd{f}\|_{\mathrm{BL}}^2=\sum_i|f_i\|_{\mathrm{BL}}^2.$ Denote $\bd{g}(\bd{x}, \bd{y})=\nabla_{\bd{x}} \log p(\bd{x})k(\bd{x},\bd{y})+\nabla_{\bd{x}} k(\bd{x},\bd{y}).$ We assume $\|\bd{g}(\bd{x}, \bd{y})\|_{\mathrm{BL}}<\infty.$ We define the Lipschitz metric between measures $\mu$ and $\nu$ as follows,
$$\mathrm{BL}(\mu, \nu)=\sup_f{\mathbb{E}_\mu f-\mathbb{E}_\nu f, \quad \textit{s.t.}\quad \|f\|_{\mathrm{BL}}\le 1}.$$
 Similar to the theoretical result of $\widetilde{\mu}^j_N$, we have the following result for $\hat{\mu}^j_M.$
%With mild conditions, for all bounded $h$, the theoretical result of SVGD indicates that $\mathbb{E}_{\widetilde{\mu}^j_N}[h]\rightarrow \mathbb{E}_{\mu^j_{\infty}}[h],$ which means that empirical measure $\widetilde{\mu}^j_N$ weakly converges to $\mu^j_{\infty}.$ Denote $\bd{g}(\bd{x}, \bd{y})=\nabla_{\bd{x}} \log p(\bd{x})k(\bd{x},\bd{y})+\nabla_{\bd{x}} k(\bd{x},\bd{y}).$ S
\begin{thm}
\label{concen}
Suppose $\{\bd{z}^0_i\}_{i=1}^N$ and $\{\bd{y}^0_i\}_{i=1}^M$ are drawn from the distribution with probability measure $\mu_{\infty}^0$ and density function $q_0$, where $q_0$ is log-concave, such as Gaussian distribution. Assume
\begin{equation*}
\lim_{N\rightarrow\infty}\mathrm{BL}(\widetilde{\mu}^0_N, \mu_{\infty}^0)=0, \quad \lim_{M\rightarrow\infty}\mathrm{BL}(\hat{\mu}^0_M, \mu_{\infty}^0)=0,
\end{equation*}
then for $j=1,2,\cdots, K$ and bounded continuous function $h$, we have
$$\sqrt{M}(\mathbb{E}_{\hat{\mu}^j_M}[h]-\mathbb{E}_{\mu^j_{\infty}}[h])\rightarrow \mathcal{N}(0, \sigma^2),$$
\end{thm}
where $\mathcal{N}(0, \sigma^2)$ is normal distribution with variance $\sigma^2$.
The proof of theorem~\ref{concen} can be found on appendix. Theorem~\ref{concen} indicates particles $\{\bd{y}^j_i\}_{i=1}^M$ with empirical measure $\hat{\mu}^j_M$ and empirical density $\{\hat{q}_j(\bd{y}^j_i)\}_{i=1}^M$ satisfy the concentration property~\citep{spohn2012large}. The convergence rate of $\{\bd{y}^j_i\}_{i=1}^M$ is $O(1/\sqrt{M}).$

%Equation \eqref{optinball} indicates that with mild conditions, $$\KL(q_{j+1}, p)-\KL(q_j, p)\le -\frac{\epsilon}{2}\mathbb{D}(q_j, p),$$
%which means that at iteration $j,$ the transformed distribution $q_{j+1}$ has smaller $\KL$ divergence with target distribution $p$ than that of $q_{j}$ by at least $\frac{\epsilon}{2}\mathbb{D}(q_j, p).$
In the following, we provide some analysis on the convergence property of our importance proposal $q_K$ to the target distribution $p.$ If we take $\epsilon$ in the transformation defined in \eqref{transform} to be infinitesimal, the evolution equation of random variable reduces to a partial differential equation(PDE),
\begin{equation}
\label{part}
\frac{d\bd{z}^t}{dt}=\mathbb{E}_{\bd{x}\sim{q_t}}[\nabla_{\bd{x}} \log p(\bd{x})k(\bd{x},\bd{z}^t)+\nabla_{\bd{x}} k(\bd{x},\bd{z}^t)].
\end{equation}
Here we use $\bd{z}^t$ to denote the evolved particle at current time $t$ with density function $q_t.$  PDE\eqref{part} captures one type of Vlasov process for interacting particles system~\citep{braun1977vlasov}. Based on the continuous-time Vlasov process, the convergence rate of $q_K$ to $p$ can be more conveniently illustrated.

\begin{thm}
\label{thm2}
Suppose random variable $\bd{z}^t$ is the solution of PDE \eqref{part},
then the probability density function of $\bd{z}^t$, denoted by $q_t$, satisfies the following PDE,
\begin{equation}
\label{diffode}
\frac{\partial q_t}{\partial t}=-\mathrm{div}(q_t\mathbb{E}_{\bd{x}\sim{q}}[\nabla_{\bd{x}} \log p(\bd{x})k(\bd{x},\bd{z})+\nabla_{\bd{x}} k(\bd{x},\bd{z})]).
\end{equation}
where $\mathrm{div}$ denotes the divergence of a vector.%$\mathrm{div}\boldsymbol{f}(x)=\sum_{i=1}^d\frac{\partial f_i}{\partial x_i}.$
\end{thm}
The proof of theorem \ref{thm2} can be found on appendix, which is different from the proof provided in the theoretical proof of SVGD and more general than that. It builds a general connection between the evolution of random variable and the evolution of its density function. Theorem~\ref{thm2} helps us establish one importance property of $q_t$ in our algorithm, provided in the following algorithm.
\begin{lem}
\label{lemma1}
The evolution equation of the density function $q_t$ satisfies the following PDE,
\begin{equation}
\label{klksd}
\frac{d\mathrm{KL}(q_t\mid\mid p)}{dt}=-\mathbb{D}(q_t,p),
\end{equation}
where $\mathbb{D}(q_t,p)$ is the KSD between density functions $q_t$ and the target density $p$.
\end{lem}
Lemma~\ref{klksd} indicates that the KL divergence between the iteratively transformed distribution and the target distribution $p$ is monotone decreasing w.r.t. time.
If the relationship $ \mathrm{KL}(q_t\mid\mid p) \le \frac{1}{\gamma} \mathbb{D}(q_t,p)$ can be established, $0<\gamma<\infty$, we have the following convergence of $q_t,$
\begin{equation}
\label{converg}
\KL(q_t, p)\le C \exp(-\gamma t).
\end{equation}
Equation (\ref{converg}) indicates that the KL divergence between the evolved density $q_t$ and the target density $p$ has exponential decay. Although it is unclear whether $\gamma$ satisfies $0<\gamma<\infty$ in general cases, numerical experiments on Gaussian mixture models(GMM) have demonstrated that we have $\KL(q_t, p)\le C \exp(-\gamma t)$ in this case when the initial distribution $q_0$ is Gaussian distribution.

\fi
\section{A PATH INTEGRATION METHOD}
% \section{\normalsize{A PATH INTEGRATION METHOD}}
% \section{A Path Integration Method}
\begin{algorithm}[tb]
\caption{SVGD with Path Integration for estimating $\KL(q_0 ~||~p)$ and $\log Z$}
\label{ksdalgo}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Target distribution $p(x) = \bar p(x)/Z$; an initial distribution $q_0$.
\STATE {\bfseries Goal:} Estimating $\KL(q_0\mid\mid p)$ and the normalization constant $\log Z.$
%denote $H(\theta,\eta) = -\nabla_{[\theta,\eta]}^2 \log p({\theta},{\eta}|{X})$; budget size $\mk$.
\STATE{ Initialize $\hat K =0.$ Initialize particles $\{\vx_i^0\}_{i=1}^n\sim q_0(\bd{x}).$}
\STATE{Compute $\hat{\mathbb{E}}_{q_0}[\log(q_0(\vx)/\overline{p}(\vx))]$ via sampling from $q_0.$}
%\FOR{$j=1,2,\cdots,K$}
\WHILE{iteration $\ell$}
\STATE %{Calculate $\vx^j_i=\hat{\bd{T}}_j(\vx^{j-1}_i)$ for $i=1,2,\cdots N.$ }
$$
\hat K \gets \hat K + \epsilon  \hat{\mathbb{D}}({q}_\ell ~||~ p)^2,
$$
$$\vx_i^{\ell+1} \gets \vx_i^\ell + \bd{\phi}_{\ell +1}(\vx_i^\ell), $$
%\STATE%{Calculate $\hat{\mathbb{D}}\leftarrow\hat{\mathbb{D}}+\epsilon \hat{\mathbb{D}}(\widetilde{q}_j,p)$ via equation \eqref{empiricalksd}.}
where $\hat{\mathbb{D}}({q}_\ell ~||~ p)$ is defined in \eqref{equ:hats}.
%\STATE{j=j+1.}
\ENDWHILE
%\STATE{Calculate $\hat{\mathbb{E}}[\log(q_0(x)/\overline{p}(x))]$ by drawing a set of samples $\{x_i\}\sim q_0(x).$}
\STATE {Estimate $\KL(q_0 ~||~  p)$ by $\hat K$ and $\log Z$ by $\hat{\mathbb{D}} - \hat{\mathbb{E}}_{q_0}[\log(q_0(\vx)/\overline{p}(\vx))].$}
%the following M-estimator, $$\boldsymbol{\hat{\theta}}_{\KL-W}=\argmax_{\boldsymbol{\theta}\in\Theta}\sum_{k=1}^d\frac1n\sum_{j=1}^n\frac{p(\boldsymbol{\widetilde{x}}_j^k| \boldsymbol{\hat{\theta}}_k)}{p(\boldsymbol{\widetilde{x}}_j^k| \boldsymbol{\widetilde{\theta}}_k)}\log p(\boldsymbol{\widetilde{x}}_j^k| \boldsymbol{\theta}).$$
\end{algorithmic}
\end{algorithm}

We mentioned that the original SVGD
does not have the ability to estimate the partition function. 
Section 3 addressed this problem by 
%We address this problem by 
turning SVGD into a standard importance sampling algorithm in Section 3.
%There is an alternative way
Here we introduce another method
for estimating KL divergence and normalization constants that is more directly motivated by the original SVGD,
by leveraging the
fact that the Stein discrepancy is a type of gradient of KL divergence.
This method does not need to estimate the importance weights but has to run SVGD to converge to diminish the Stein discrepancy between intermediate distribution $q_\ell$ and $p$. In addition, this method does not perform as well as Algorithm 1 as we find empirically.
Nevertheless, we find this idea is conceptually interesting and useful to discuss it.
%but tends to perform worse
%than the one based on importance weights,
%that is more directly motivated by the original SVGD.
%we address the

%To be specific, recall that from \eqref{vgddecrease} in Section~\ref{sec:stein}\todo{sec:2.1},
Recalling Equation {\eqref{vgddecrease}} in Section 2.1, we know that
if we perform transform $\T(\vx) = \vx +  \epsilon \ff^*(\vx)$ with $\ff^*$ defined in \eqref{transf},
the corresponding decrease of KL divergence would be
\begin{align}
\begin{split}
 \KL(q ~||~ p)  - \KL(\T\sharp q  ~||~ p)
&  \approx \epsilon \cdot || \ff^* ||_\H \cdot \S(q ~|| ~ p)  \\
&  \approx \epsilon \cdot \S(q ~|| ~ p)^2,
\end{split}
\label{def:kldecrease}
\end{align}
where we used the fact that $\S(q~||~p) = ||\ff^*||_\H$, shown in \eqref{equ:sdefine}.
Applying this recursively on $q_\ell$ in \eqref{def:kldecrease}, we get
$$
 \KL(q_0 ~||~ p) - \KL(q_{\ell+1} ~||~ p)  \approx \sum_{\jmath = 0}^\ell
\epsilon \cdot \S(q_{\jmath} ~|| ~ p)^2.
$$
Assuming $\KL(q_{\ell} ~||~ p) \to 0$ when $\ell \to \infty$,
we get
\begin{equation}
\label{klestimate}
\KL(q_0 ~||~ p)  \approx \sum_{\ell = 0}^\infty
\epsilon \cdot \S(q_{\ell} ~|| ~ p)^2.
\end{equation}

By \eqref{equ:sdefine}, the square of the KSD can be empirically estimated via V-statistics, which is given as
\begin{align}\label{equ:hats}
\hat \S(q_{\ell} ~|| ~ p)^2 = \frac{1}{n^2}\sum_{i,j=1}^n \kappa(\vx_i^\ell, \vx_j^\ell).
\end{align}
%where $\{\}$
Overall, equation~\eqref{klestimate} and \eqref{equ:hats} give an estimator of the KL divergence between $q_0$ and $p = \bar p(\bd{x})/Z.$
This can be transformed into an estimator of the log normalization constant $\log Z$ of $p$, by noting that
\begin{equation}
\log Z=\KL(q_0\mid\mid p)-\mathbb{E}_{q_0}[\log(q_0(\vx)/\overline{p}(\vx))],
\end{equation}
where the second term can be estimated by drawing a lot of samples to diminish its variance since the samples from $q_0$ is easy to draw. %$\hat{\mathbb{E}}_{q_0}[\log(q_0(\vx)/\overline{p}(\vx))]=\frac{1}{N}\sum_{i=1}^N\log(q_0(\vx_i)/\overline{p}(\vx_i)), $ where $\bd{x}_i\sim q_0$ and $N$ is large.
%See Algorithm~\ref{ksdalgo} for the
The whole procedure is summarized in Algorithm~\ref{ksdalgo}.

%Assume $q_t$ approximates

%We will leverage this fact to develop a path integration for estimating KL divergence in Section~\ref{sec:pathintegration}\todo{fix ref}.  With some insight of equation \eqref{klksd}, we propose a new algorithm which can be applied to evaluate the KL divergence between $q_0$ and the unnormalized distribution $p(\bd{x}),$ and its partition functions. Rewrite equation \eqref{klksd} in the integration form,
%\begin{equation}
%\label{sumksd}
%\KL(q_t, p)=\KL(q_0, p)-\int_0^t \mathbb{D}(q_s, p)ds.
%\end{equation}
%If $\KL(q_t, p)\rightarrow 0$ can be established (verified by most experiments), we have $\int_0^t \mathbb{D}(q_s, p)ds\rightarrow \KL(q_0, p)$ as $t\rightarrow\infty.$ Replace the integration of equation (\ref{sumksd}) with summations over $\mathbb{D}(q_j,p)$  in each iteration of our algorithm and we notice that $\mathbb{D}(q_j,p)$ can be empirically estimated via V-statistics:
%\begin{equation}
%\label{empiricalksd}
%\hat{\mathbb{D}}(\widetilde{q}_j,p)=\frac{1}{N^2}\sum_{z_i,z_l\sim \widetilde{q}_j} \kappa_p(z_i,z_l),
%\end{equation}
%where $\kappa_p(\cdot,\cdot)$ is defined in equation (\ref{ksdkernel}) and $\widetilde{q}_j$ denotes the empirical density of particles $\{z_i^j\}_{i=1}^N$. The $\KL$ divergence between $q_0$ and unnormalized $p$, $\KL(q_0\mid\mid p),$ can be estimated based on equation \eqref{sumksd} and \eqref{empiricalksd}. As a result, we can estimate the normalization constant $Z$ in the target distribution $ p(x)=\overline{p}(x)/Z$ by
%\begin{equation}
%\log Z=\KL(q_0\mid\mid p)-\mathbb{E}[\log(q_0(x)/\overline{p}(x))].
%\end{equation}
%And $\mathbb{E}[\log(q_0(x)/\overline{p}(x))]$ can be easily estimated by drawing a large set of samples $\{x_i\}_{i=1}^n$ from the simple distribution $q_0(x)$, $\hat{\mathbb{E}}[\log(q_0(x)/\overline{p}(x))]=\frac1n\sum_i \log(q_0(x_i)/\overline{p}(x_i).$ The whole procedure is summarized in algorithm \ref{ksdalgo}.
%Algorithm \ref{ksdalgo} provides us a new perspective to estimate the KL divergence between the normalized distribution $q_0$ and another unnormalized distribution $p$. Therefore, it can be naturally applied to estimate the normalization constant of $p.$ As much efforts are devoted to analyze algortihm~\ref{VarIS:algo} in this paper, more theoretical and empirical investigations of algorithm \ref{ksdalgo} are left as future work.

%\section{Time Complexity}
%In each iteration of VIS, we need $O(d*N*M+d*M^2+(d^2*M + d^3)*N)$ where $M$ is the number of particles for approximating the mapping and $N$ is the number of particles for importance sampling. In each iteration of AVIS, we need $O(d*N^2+(d^2*N + d^3)*N).$ In HAIS, suppose we do $L$ leapfrog step, we have $O(L*N*d).$

